TopoBench: Benchmarking LLMs on Hard Topological Reasoning

Solving topological grid puzzles requires reasoning over global spatial invariants such as connectivity, loop closure, and region symmetry and remains challenging for even the most powerful large language models (LLMs). To study these abilities under controlled settings, we introduce TopoBench, a benchmark of six puzzle families across three difficulty levels. We evaluate strong reasoning LLMs on TopoBench and find that even frontier models solve fewer than one quarter of hard instances, with two families nearly unsolved. To investigate whether these failures stem from reasoning limitations or from difficulty extracting and maintaining spatial constraints, we annotate 750 chain of thought traces with an error taxonomy that surfaces four candidate causal failure modes, then test them with targeted interventions simulating each error type. These interventions show that certain error patterns like premature commitment and constraint forgetting have a direct impact on the ability to solve the puzzle, while repeated reasoning is a benign effect of search. Finally we study mitigation strategies including prompt guidance, cell-aligned grid representations and tool-based constraint checking, finding that the bottleneck lies in extracting constraints from spatial representations and not in reasoning over them. Code and data are available at github.com/mayug/topobench-benchmark.

==> related_papers.tex <==
https://arxiv.org/pdf/2407.14790v1
https://arxiv.org/pdf/2505.14552
https://arxiv.org/pdf/2402.11291
https://arxiv.org/pdf/2505.19914

https://arxiv.org/pdf/2506.02867
https://arxiv.org/pdf/2505.16381 position encoding

==> sections/benchmark.tex <==
\section{Benchmark and Methodology}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/introduction/figure1.png}
\caption{TopoBench Overview}
\label{fig:topobench}
\end{figure}

\label{sec:benchmark}
We introduce TopoBench, a puzzle-solving benchmark that targets \emph{topological} and \emph{spatial} reasoning in language models. Unlike existing puzzle-based evaluations that center on arithmetic constraints (Sudoku, Keen) or local pattern matching (Mines, Mosaic), TopoBench requires models to maintain and update global spatial invariants---path connectivity, region partitioning, visibility propagation---through purely textual interaction, without external code execution. The benchmark comprises six puzzle families spanning three difficulty tiers (easy, medium, hard), and is designed so that even frontier reasoning models achieve low accuracy on hard instances (e.g., ${\sim}0.25$ for GPT-5-mini; ${\sim}0.10$ for Gemini-3-Flash).

\paragraph{Task Families.}

We select six puzzle families, five from the Simon Tatham Portable Puzzle Collection and one (Flow Free) generated separately, each targeting a distinct feature of topological and geometric reasoning:

\begin{itemize}[leftmargin=*,itemsep=2pt]
    \item \textbf{Flow Free} --- Route non-intersecting paths between color-matched endpoints, filling every cell. Tests \emph{Path Connectivity}.
    \item \textbf{Bridges (Hashiwokakero)} --- Connect numbered islands via horizontal/vertical bridges so each island's count matches its number, no bridges cross, and all islands form one connected component. Tests \emph{Network Connectivity}.
    \item \textbf{Galaxies (Tentai Show)} --- Partition a grid into regions, each rotationally symmetric around a marked center. Tests \emph{Rotational Symmetry}.
    \item \textbf{Undead} --- Place monsters (ghosts, vampires, zombies) on a grid with mirrors so line-of-sight counts match given clues, with visibility rules depending on monster type. Tests \emph{Reflection}.
    \item \textbf{Pattern (Nonogram)} --- Reconstruct a binary grid from row/column clues specifying consecutive filled-cell run lengths. Tests \emph{Contiguity and Adjacency} across intersecting axes.
    \item \textbf{Loopy (Slitherlink)} --- Draw a single closed loop on grid edges so numbered cells' edge counts match their clue. Tests \emph{Loop Closure} subject to local constraints.
\end{itemize}

\paragraph{Dataset Construction.}

All instances are generated algorithmically. The five Tatham-family puzzles use the collection's built-in generators; Flow Free uses a separate algorithmic pipeline. Each family includes three difficulty tiers that scale in complexity and board size. The dataset contains 50 samples per puzzle per tier.

\paragraph{Human reference.}
The PUZZLES benchmark reports that a human expert solves 100\% of puzzles at their easiest-human presets~\citep{estermann2024puzzles}.
TopoBench's easy tier uses comparable or lower difficulty settings, meaning these instances are straightforward for experienced human solvers.
This contextualizes the models' low easy-tier accuracy: puzzles that humans find routine remain difficult for most models we evaluate.

\paragraph{Evaluated Models.}

We evaluate nine reasoning-oriented models spanning closed- and open-source families, autoregressive and diffusion-based architectures, dense and mixture-of-experts parameterizations, and scales from 17B active to 671B total parameters. Table~\ref{tab:models} summarizes the lineup. We focus on reasoning-capable models because TopoBench's multi-step spatial inference under high state-tracking load pushes non-reasoning models to near-zero accuracy on medium and hard tiers. Models were selected for (i)~strong performance on established reasoning benchmarks (AIME, MATH, ARC-AGI).

\begin{table}[t]
\centering
\small
\caption{Models evaluated on TopoBench. \emph{Active} denotes active parameters for MoE models. Architecture: D\,=\,dense, MoE\,=\,mixture-of-experts, Diff\,=\,diffusion.}
\label{tab:models}
\begin{tabular}{llccccl}
\toprule
\textbf{Model} & \textbf{Source} & \textbf{Params (Active)} & \textbf{Arch.} & \textbf{Open} & \textbf{Think} & \textbf{Multimodal} \\
\midrule
GPT-5-mini              & OpenAI    & --              & D     & --  & \checkmark & \checkmark \\
Gemini-3-Flash-Preview  & Google    & --              & --    & --  & \checkmark & \checkmark \\
DeepSeek-v3.2           & DeepSeek  & 671B (37B)      & MoE   & \checkmark & \checkmark & -- \\
Qwen3-32B               & Alibaba   & 32B             & D     & \checkmark & \checkmark & -- \\
OLMo-3.1-32B-Think      & AI2       & 32B             & D     & \checkmark & \checkmark & -- \\
LLaMA-4-Maverick        & Meta      & 400B (17B)      & MoE   & \checkmark & --         & -- \\
Mercury                 & Inception & --              & Diff  & \checkmark & --         & -- \\
GLM-4.7-Flash           & Zhipu AI  & --              & --    & \checkmark & --         & -- \\
GPT-OSS-120B             & OpenAI    & 120B             & D     & \checkmark & \checkmark & -- \\
\bottomrule

\end{tabular}
\end{table}


\paragraph{Prompting.}
Each prompt contains (i)~a complete rule specification for the puzzle family, and (ii)~one worked example showing input and final solution only---no intermediate reasoning traces---so that models must derive their own strategy from the rules. We allow up to \textbf{100k tokens} per evaluation to accommodate extended chains of thought.

\paragraph{Execution.}
We evaluate models using single-attempt (pass@1) scoring. All models run with default decoding hyperparameters; thinking mode is activated at the highest level where supported. Some models are accessed via OpenRouter, with providers pinned for reproducibility. Crucially, \emph{no external code execution is permitted}: we measure reasoning in the CoT alone, not the ability to offload computation to external solvers.

\paragraph{Verification.}
Each puzzle type has a dedicated constraint-checking verifier. The five Tatham puzzles are verified by the collection's original C-based solvers and Flow Free by a separate verifier.
Verification is binary (correct/incorrect) with no partial credit. Models output a parseable JSON grid encoding their solution; the verifier reconstructs the proposed grid and checks it against the full constraint set. We parse the json outputs as leniently as possible.


==> sections/benchmark_old.tex <==
\section{Benchmark and Methodology}
\label{sec:benchmark}

We introduce TopoBench, a puzzle-solving benchmark designed to test \emph{topological} and \emph{spatial} reasoning in language models under realistic constraints: no external code execution, a purely textual interface, and large-context prompts that include complete rule specifications. The benchmark comprises six puzzle families---\emph{Flow Free}, \emph{Bridges}, \emph{Galaxies}, \emph{Undead}, \emph{Pattern}, and \emph{Loopy}---spanning three difficulty tiers (easy, medium, hard). In this section we describe the task families, their selection rationale, the input encodings, prompting protocol, evaluation models, and the verification pipeline.

\subsection{Task Families}
\label{subsec:puzzle-families}

Each puzzle family targets a distinct topological reasoning phenomenon (as defined in \citet{giadikiaroglou2024puzzlesurvey} survey), requiring the solver to maintain and update global spatial invariants rather than apply purely local rules:
\begin{itemize}
    \item \textbf{Flow Free:} the solver must route non-intersecting paths between color-matched endpoints on a grid, filling every cell exactly once. This stresses path connectivity reasoning and non-crossing constraint maintenance across the entire board.
    \item \textbf{Bridges (Hashiwokakero):} numbered islands on a grid must be connected by horizontal or vertical bridges such that each island's bridge count matches its number, no bridges cross, and all islands form a single connected component. This requires adjacency reasoning, degree-constraint satisfaction, and global connectivity verification.
    \item \textbf{Galaxies (Tentai Show):} the grid must be partitioned into regions, each rotationally symmetric around a marked center dot. This demands symmetry detection and region partitioning under a global constraint that every cell belongs to exactly one region.
    \item \textbf{Undead:} monsters (ghosts, vampires, zombies) must be placed on a grid with mirrors such that line-of-sight counts along rows and columns match given clues. Ghosts are invisible in mirrors, vampires are invisible directly, and zombies are always visible. This involves geometric propagation through reflections and visibility constraint tracking.
    \item \textbf{Pattern (Nonogram):} row and column clues specify the lengths of consecutive filled-cell runs. The solver must reconstruct a binary grid satisfying all clues simultaneously, requiring joint reasoning over intersecting row and column constraints.
    \item \textbf{Loopy (Slitherlink):} numbered cells indicate how many of their four edges belong to a single closed loop that must be drawn on the grid without crossings or branches. This tests global loop formation subject to local edge-count constraints.
\end{itemize}

\subsection{Puzzle Selection Rationale}
\label{subsec:puzzle-selection}

Five of our six puzzle families are sourced from the Simon Tatham Portable Puzzle Collection; Flow Free is generated separately. We selected these families based on three criteria that distinguish TopoBench from existing puzzle-based evaluations.

\paragraph{Topological and structural reasoning.}
Following the taxonomy of~\citet{giadikiaroglou2024puzzlesurvey}, our puzzles require topological or structural reasoning---path connectivity (Flow Free, Loopy), region partitioning and symmetry (Galaxies), degree constraints with global connectivity (Bridges), visibility propagation through reflections (Undead), and joint row--column constraint satisfaction (Pattern)---rather than arithmetic constraint satisfaction. This distinguishes them from arithmetic puzzles (Sudoku, Keen, Towers), sequential/motion puzzles (Fifteen, Twiddle), and local-only constraint puzzles (Mines, Mosaic) in the broader Tatham collection.

We selected six puzzle families from the Simon Tatham Portable Puzzle Collection (except for flow free) based on three objective criteria that distinguish our benchmark from existing puzzle-based evaluations. 

\paragraph{Topological and Structural Reasoning.}
 Flow Free requires maintaining multiple non-intersecting paths; Loopy demands a single connected loop; Galaxies requires region symmetry verification; Bridges needs network connectivity checking. This property stresses models' state tracking capabilities more than puzzles with local constraints.

\subsection{Instance Generation and Dataset Composition}
\label{subsec:instance-generation}

All puzzle instances are generated algorithmically. Five families (Bridges, Galaxies, Undead, Pattern, Loopy) use the generators from the Simon Tatham Portable Puzzle Collection, which produce instances with unique solutions by construction. Flow Free instances are generated using a separate algorithmic pipeline (WHICH ONE?). Each puzzle family includes instances at three difficulty tiers---easy, medium, and hard---corresponding to increasing board sizes that progressively raise the burden of global constraint management and state tracking. We evaluate 20 instances per puzzle type per difficulty tier, yielding a total of $6 \times 3 \times 20 = 360$ puzzle instances. Board sizes increase with difficulty, but the exact dimensions are not fixed across instances: the generators produce puzzles of varying sizes within a target range for each tier (e.g., Bridges uses approximately $5{\times}5$ at easy, $7{\times}7$ at medium, and $10{\times}10$ at hard; other families follow analogous progressions).



\subsection{Prompting Protocol}
\label{subsec:prompting}

For each puzzle instance, the prompt includes: (i) a complete specification of the puzzle family's rules, and (ii) a single worked example instance from the same family demonstrating the input and expected output format. To avoid leaking intermediate reasoning strategies that could inflate performance, the worked example provides only the puzzle input and final solution---it does \emph{not} include step-by-step reasoning traces. Models must derive their own solution strategy from the rules alone.

We set a maximum context budget of up to \textbf{100k tokens} per evaluation to allow complete rule descriptions, rich input encodings, and sufficient space for models to deliberate on difficult instances. Chains of thought produced by reasoning models on hard puzzles typically range from x to y tokens. The model is instructed not to ask clarifying questions and to solve the puzzle with the information provided.

\subsection{Model Selection}
\label{subsec:model-selection}

We evaluate a diverse set of reasoning-oriented language models, spanning both closed-source and open-source families. We focus on reasoning-oriented models because the benchmark is intentionally difficult and aims to probe multi-step spatial inference under high state-tracking load; non-reasoning models are expected to perform near zero on medium and hard tiers.

We select models based on two criteria: (i) strong performance on established reasoning benchmarks (e.g., AIME, MATH, ARC-AGI), indicating that the model has been optimized for or is capable of multi-step deliberation; and (ii) coverage of the current model landscape, spanning closed-source and open-source families, different scales, and distinct architectural choices. Table~\ref{tab:models} summarizes the evaluated models.

\paragraph{Closed-source models.}
We evaluate three frontier closed-source reasoning models.
\textbf{GPT-5-mini}~\citep{gpt5systemcard} is OpenAI's compact reasoning model, which supports both text and vision inputs and uses high reasoning effort for all evaluations.
\textbf{Gemini-3-Flash-Preview}~\citep{team2023gemini} is Google's efficient reasoning model from the Gemini family, supporting text, image, and structured inputs.
\textbf{DeepSeek-v3.2}~\citep{deepseekv3} is DeepSeek's latest mixture-of-experts model with 671B total parameters (37B active), trained with multi-token prediction and exhibiting strong reasoning capabilities. DeepSeek-v3.2 also exposes its full chain of thought, making it the primary target for our error analysis (Section~\ref{sec:error_analysis}).

\paragraph{Open-source models.}
We evaluate seven open-source or openly accessible models spanning a range of architectures and scales.
\textbf{Qwen3-32B}~\citep{qwen3} is Alibaba's 32B-parameter dense reasoning model supporting both ``thinking'' and non-thinking modes; we evaluate in thinking mode.
\textbf{Qwen3-VL-235B-A22B}~\citep{qwen3} is the vision-language variant of Qwen3 with 235B total parameters (22B active) in a mixture-of-experts architecture, evaluated in thinking mode with vision inputs where applicable.
\textbf{OLMo-3.1-32B-Think}~\citep{olmo2} is AI2's 32B-parameter reasoning model from the fully open OLMo family, designed for transparent and reproducible research.
\textbf{LLaMA-4-Maverick-17B-128E-Instruct}~\citep{llama4} is Meta's natively multimodal Maverick variant with 17B active parameters across 128 experts, from the LLaMA~4 family.
\textbf{Mercury}~\citep{mercury2025} is a diffusion-based language model from Inception Labs that generates multiple tokens in parallel, representing an architecturally distinct alternative to autoregressive transformers.
\textbf{GLM-4.7-Flash}~\citep{glm4} is Zhipu AI's efficient model from the GLM-4 family, designed for fast inference.
\textbf{GPT-OSS-20B} is a 20B-parameter open-source reasoning model from OpenAI.

The selection represents a broad cross-section of the current model landscape: autoregressive and diffusion-based architectures; dense and mixture-of-experts parameterizations; scales from 17B active parameters to 671B total; and both text-only and multimodal capabilities. Compared to the models typically evaluated in existing puzzle benchmarks such as KORGym~\citep{shi2025korgym} and Enigmata~\citep{chen2025enigmata2025}, our model set is more recent and skewed toward reasoning-oriented variants, reflecting TopoBench's focus on challenging multi-step spatial inference.

\begin{table}[t]
\centering
\small
\caption{Models evaluated on TopoBench. ``Active'' denotes active parameters for MoE models. Representations: A = ASCII, I = IntFormat, J = IntFormat-JSON, V = ASCII+image.}
\label{tab:models}
\begin{tabular}{llccl}
\toprule
\textbf{Model} & \textbf{Source} & \textbf{Params (Active)} & \textbf{Open} & \textbf{Repr.} \\
\midrule
GPT-5-mini              & OpenAI    & undisclosed      & No  & A, I, J, V \\
Gemini-3-Flash-Preview  & Google    & undisclosed      & No  & A, I, J, V \\
DeepSeek-v3.2           & DeepSeek  & 671B (37B)       & Yes$^\dagger$ & A, I \\
Qwen3-32B               & Alibaba   & 32B              & Yes & A, I \\
Qwen3-VL-235B-A22B      & Alibaba   & 235B (22B)       & Yes & A \\
OLMo-3.1-32B-Think      & AI2       & 32B              & Yes & A, I \\
LLaMA-4-Maverick        & Meta      & 400B (17B)       & Yes & A, I \\
Mercury                 & Inception & undisclosed      & Yes & A, I \\
GLM-4.7-Flash           & Zhipu AI  & undisclosed      & Yes & A, I \\
GPT-OSS-20B             & OpenAI    & 20B              & Yes & A, I \\
\bottomrule
\multicolumn{5}{l}{\footnotesize $^\dagger$Weights available; API-based evaluation.}
\end{tabular}
\end{table}

\subsection{Experimental Protocol}
\label{subsec:experimental-protocol}

Each model is evaluated on 50 instances per puzzle type per difficulty tier. For models supporting multiple representations, we evaluate each representation independently, yielding separate accuracy scores per (model, puzzle, difficulty, representation) tuple. All evaluations use a single attempt per instance (pass@1) with a maximum token budget of 100k tokens.

We use default decoding hyperparameters for each model and activate thinking mode on all models that support it on the highest level.
Models were run via different apis, some of them via openrouter. to keep reporducibility we pin the model providers on openrouter.

\paragraph{No code execution.}
Unlike other puzzle-solving evaluations that permit program execution or implicitly reward tool use, we disallow external code execution in all conditions. The goal is to measure \emph{reasoning from the prompt alone}---the model's ability to maintain and update spatial state through its chain of thought---rather than the ability to offload computation to external solvers.

\subsection{Verification Pipeline}
\label{subsec:verification}

Each puzzle type has a dedicated constraint-checking verifier that determines correctness of the model's output. For the five Tatham-collection puzzles, verification is performed by the original C-based solvers from the Tatham collection, which check all puzzle constraints exhaustively (e.g., loop closure and edge counts for Loopy; connectivity, degree satisfaction, and non-crossing for Bridges; row/column run counts for Pattern [IS THAT TRUE???]). The Flow Free verifier checks path completeness, endpoint matching, non-crossing, and full grid coverage [IS THAT TRUE?]. All verification is binary (correct/incorrect); we do not award partial credit.

In addition to final-answer verification, we extract and evaluate intermediate metrics: (i) \emph{board extraction rate}---whether the model's output contains a parseable board in the expected format; and (ii) \emph{structural validity rate}---whether the extracted board has the correct dimensions and respects the puzzle's fixed cells (i.e., the starting board is not modified). These intermediate metrics help distinguish formatting failures from reasoning failures. [DO WE WANT TO REPORT THESE?]

The output format is consistent across all puzzle types: models are instructed to produce a parseable JSON object containing a grid representation that encodes their proposed solution state. This uniform output schema simplifies automated extraction and verification. The verifier parses the JSON, reconstructs the proposed grid, and checks it against the full set of puzzle-specific constraints.

We try to be as lenient as possible for the format as long as it is still parseable



\subsection{Positioning Relative to Prior Work}
\label{subsec:positioning}

TopoBench differs from existing puzzle benchmarks in several respects. Our instances are substantially harder than those used in prior evaluations: on the hard tier, even the best closed-source models achieve low aggregate accuracy (approximately 0.25 for GPT-5-mini; 0.10 for Gemini-3-Flash), while open-source models are near zero.












 























==> sections/diagnosis.tex <==
\section{Diagnosing Failure Modes}
\label{sec:diagnosis}
\label{sec:error_analysis}
\label{sec:interventions}

To understand \emph{why} models fail on topology-heavy reasoning, we perform a systematic error analysis on full chains of thought, then design targeted interventions to test which failure modes are genuine causal drivers.
We focus on DeepSeek-v3.2, the most competent reasoning model in our evaluation that exposes its complete chain of thought (14,000--42,000 tokens per puzzle).

\paragraph{Observational method.}
Following prior LLM-as-a-judge evaluation protocols~\citep{g_eval,prometheus}, we use GPT-5-mini to label each chain of thought with a small set of error categories.
We develop these categories iteratively: first, we run a coarse pass over chains of thought to surface prevalent behavioral patterns; we then manually curate and define a taxonomy of eleven failure modes (Table~\ref{tab:error_taxonomy_judge}); finally, the judge tags each chain of thought with up to three labels.
To facilitate manual verification, the judge also returns the neighboring 15 characters around each identified error location.
The prompt is provided in Appendix~\ref{app:judge_prompt}. (need to add human verified that the judgements are correct)
We analyze 750 traces in total: 5 puzzle types $\times$ 3 difficulty tiers $\times$ 50 traces each.

\input{sections/table_error_types_judge_v2}

\paragraph{Observational results.}
Figure~\ref{fig:error_trio} summarizes the prevalence of each error type across difficulty tiers, both aggregated across all five puzzle types (left) and broken down for the two puzzles on which we later run interventions: Bridges (center) and Undead (right).
Per-puzzle breakdowns for all five families are provided in Appendix~\ref{app:per_puzzle_errors}.
Several findings stand out.

\emph{Explicit surrender dominates and scales sharply with difficulty.}
ES is by far the most prevalent behavior, rising from 28\% of traces at easy to 48\% at medium and 65\% at hard.
Bridges, the easiest puzzle in our suite, has near-zero ES across all difficulties, while other puzzles such as Galaxies reach saturation even at medium (Appendix~\ref{app:per_puzzle_errors}).
We hypothesize that explicit surrender is \emph{symptomatic} of failure rather than causal: the model recognizes it has entered a degraded reasoning state and gives up, rather than the surrender itself causing the failure.
Incomplete output (IO) follows a similar pattern, rising sharply at hard (34\% aggregate, driven by Bridges at 60\% and Galaxies at 72\%), and likewise reflects the model failing to produce a parseable answer rather than a specific reasoning error.

\emph{Premature commitment scales sharply with difficulty.}
PC nearly triples from 12\% at easy to 20\% at medium and 32\% at hard.
When the search space is large, committing early to a wrong configuration is difficult to recover from: the model wastes its token budget exploring a dead-end branch, and the accumulated context makes it harder to backtrack effectively.
Undead shows a sharp jump to 44\% PC at hard, while Bridges remains low (6\%), consistent with its simpler constraint structure.

\emph{State-tracking failure jumps at hard.}
STF nearly triples from 6\% at easy to 16\% at hard.
Larger grids overwhelm the model's ability to maintain an accurate internal representation of the board: the claimed state diverges from the cumulative effect of the model's own stated actions.
Undead exhibits the sharpest STF scaling (4\% $\rightarrow$ 10\% $\rightarrow$ 32\%), reflecting the richer state involving monster types and visibility constraints.

\emph{Repeated reasoning peaks at medium then declines.}
RR rises from 22\% at easy to 26\% at medium, then drops to 18\% at hard.
Bridges has near-zero RR across all difficulties.
The decline at hard coincides with the sharp rise in ES---the model surrenders before it has the chance to enter repetitive reasoning cycles.

\emph{Constraint forgetting is rare.}
CF drops from 7\% at easy to 2\% at hard.
Under a strict definition that requires an explicit proposed action violating structural rules (overcounting, crossing, overwriting fixed cells), constraint violations are uncommon.
The model's failures are predominantly at the reasoning level---losing track of state, committing to wrong branches, or cycling---rather than at the level of violating the puzzle's structural rules.

\emph{Representation drift is highest at easy.}
RD is most prevalent at easy and medium (30\%) and remains elevated at hard (26\%).
This aggregate trend is driven almost entirely by Pattern, which exhibits extreme RD rates far above any other puzzle type (Appendix~\ref{app:per_puzzle_errors}).
The elevated rate on easier puzzles suggests that flexible re-representation may be an adaptive strategy rather than a pure error.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/llm_judge_v2/trace_verification_main_trio_normalized.png}
\caption{Error category prevalence by difficulty tier: aggregated across all five puzzle types (left, 250 traces per tier), and broken down for Bridges (center) and Undead (right), the two puzzles targeted by our causal interventions.
Bar labels show raw counts.
ES dominates at all tiers and scales sharply with difficulty; PC and STF show pronounced increases at hard; RR peaks at medium then declines as ES rises.
Bridges exhibits near-zero ES and RR; Undead shows elevated PC and STF at hard.}
\label{fig:error_trio}
\label{fig:error_aggregated}
\end{figure}

\paragraph{Intervention setup.}
The observational analysis identifies four error types that are plausibly causal rather than symptomatic: RR, STF, CF, and PC.
To test whether these behavioral patterns genuinely drive failure, we design targeted interventions that selectively inject each error type into the model's reasoning context and measure the downstream impact on accuracy.
We evaluate DeepSeek-v3.2 on Bridges puzzles across three difficulty tiers (Easy/5$\times$5, Medium/7$\times$7, Hard/10$\times$10), with 100 puzzles per tier and 300 per condition (2,400 total API calls across 8 conditions).
Each puzzle is presented with a \emph{partial gold solution path} covering approximately 15\% of the total solution steps.
For the baseline condition, this path is unmodified; for each intervention condition, a targeted modification is applied before the model is asked to ``solve the puzzle, starting from the last state.''
All accuracy figures are reported with 95\% Wilson score confidence intervals.

To generate the raw material for interventions, we expand the puzzle solver's solution paths into partial game trees by sampling alternative moves at branching points---primarily legal-but-wrong moves such as a different bridge count on the same island pair or a connection to a different island---and following the resulting wrong paths for up to five steps until a constraint violation or engine rejection terminates the branch.
This yields both correct and incorrect branch prefixes that can be composed into intervention-specific traces.
To prevent information leakage, all candidate intervention prefixes are checked against future gold solution states; if a candidate intervention state matches any future gold state, it is discarded and a new prefix is sampled.

\paragraph{Intervention definitions.}
We define four intervention types, each targeting one causal error category from Table~\ref{tab:error_taxonomy_judge}:

\begin{itemize}[nosep]
\item \textbf{RR.}
$k{=}2$ wrong-path-then-backtrack cycles injected before the continuation point.
We test two variants: \emph{Samepoint} (wrong paths diverge from the same branching state) and \emph{Standard} (same wrong path repeated).

\item \textbf{STF.}
$k{=}3$ bridge cells independently flipped in the last three intermediate grids; the natural-language action log is left intact, creating a mismatch between the visual grid and the textual history.

\item \textbf{CF.}
One constraint violation injected at the last step, uniformly sampled from three subtypes: overcounting an island's bridge capacity, introducing an illegal bridge crossing, or modifying an island's required count.
The grid updates as if the illegal move were legal, with no error signal in the text.

\item \textbf{PC.}
The gold path prefix is replaced entirely with a wrong-path branch that diverges at the very first move and extends to half the depth of the longest available incorrect branch, with no backtrack signal.
Because the path is truncated well before the dead-end, the final state does not exhibit an obvious constraint violation.
\end{itemize}

\paragraph{Intervention results.}
Figure~\ref{fig:intervention_forest} summarizes accuracy across all conditions for both Bridges ($N{=}300$) and a cross-puzzle replication on Undead ($N{=}300$).
The shaded bands mark each puzzle's baseline accuracy.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/interventions/intervention_forest_absolute.png}
\caption{Intervention effects on Bridges (circles, $N{=}300$) and Undead (squares, $N{=}300$).
Points show total accuracy with 95\% Wilson CIs; shaded bands mark the baseline for each puzzle.
Asterisks denote conditions whose 95\% CI for $\Delta$ excludes zero.
PC and CF produce large, significant drops on both puzzles; STF reaches significance only on Undead; RR variants are indistinguishable from baseline.}
\label{fig:intervention_forest}
\end{figure}

The results reveal a clear two-tier separation.
Premature commitment ($-$20.8pp on Bridges, $-$11.3pp on Undead) and constraint forgetting ($-$10.6pp, $-$11.3pp) produce large accuracy drops that are significant on both puzzles, with confidence intervals excluding the baseline.
These two error types are the dominant causal drivers of failure.
State-tracking failure occupies a middle tier: on Bridges it produces a borderline $-$7.8pp trend (Newcombe 95\% CI upper bound $+$0.3pp), while on Undead---where the model must track a richer state involving monster types and visibility constraints---the effect strengthens to a significant $-$11.7pp.
Repeated reasoning is a null result on both puzzles: neither the Samepoint nor Standard variant differs meaningfully from baseline, and length-matched gold controls confirm that added context alone does not degrade performance.
We conclude that the repeated reasoning patterns observed in incorrect chains of thought are a \emph{symptom} of search rather than a cause of failure.

The CF result is particularly striking: constraint forgetting is among the \emph{least} prevalent error types in the observational analysis (2--7\% of traces), yet it produces a large causal effect when injected.
Correlational error frequency is thus a poor proxy for causal impact.
The contrast with STF is mechanistically informative: STF introduces a \emph{syntactic} inconsistency between the grid and the action log that the model can partially detect using the uncorrupted text, whereas CF produces an \emph{internally consistent} but semantically illegal state that requires active constraint verification---a capability the model largely lacks.
Per-difficulty breakdowns and detailed per-condition analysis are provided in Appendix~\ref{app:intervention_details}.


==> sections/diagnosis_v2.tex <==

\subsection{Diagnosing Failure Modes}
\label{sec:diagnosis}

To understand \emph{why} models fail on topology-heavy reasoning, we perform a systematic error analysis on full chains of thought, then design targeted interventions to test which failure modes genuinely drive failure.
We focus on DeepSeek-v3.2, the most competent reasoning model in our evaluation that exposes its complete chain of thought (14,000--42,000 tokens per puzzle).

\paragraph{Observational method.}
Following LLM-as-a-judge protocols~\citep{g_eval,prometheus}, we use GPT-5-mini to label each chain of thought against an error taxonomy of eleven categories, of which we focus on seven in the main body (Table~\ref{tab:error_taxonomy_judge}; full taxonomy in Appendix~\ref{app:full_error_taxonomy}).
Categories were developed iteratively: a coarse pass surfaced prevalent behavioral patterns, which we manually curated into definitions; the judge then tags each trace with up to three labels and returns neighboring characters around each error for manual verification.
The prompt is provided in Appendix~\ref{app:judge_prompt}.
We analyze 750 traces in total: 5 puzzle types $\times$ 3 difficulty tiers $\times$ 50 traces each.

\input{sections/table_error_types_judge_v2}

\paragraph{Observational results.}
Figure~\ref{fig:error_trio} summarizes error prevalence across difficulty tiers, both aggregated (left) and broken down for Bridges (center) and Undead (right).
Per-puzzle breakdowns for all five families appear in Appendix~\ref{app:per_puzzle_errors}.

Two error types scale sharply with difficulty and are plausibly causal.
Premature commitment (PC) nearly triples from 12\% at easy to 32\% at hard: committing early to a wrong configuration wastes the token budget on a dead-end branch from which the model struggles to recover.
State-tracking failure (STF) also triples (6\% $\rightarrow$ 16\%), with the sharpest increase on Undead (4\% $\rightarrow$ 32\%), whose richer state involving monster types and visibility constraints overwhelms the model's internal bookkeeping.

The remaining high-frequency categories are symptomatic rather than causal.
Explicit surrender (ES) dominates at all tiers (28\% $\rightarrow$ 65\%) but reflects the model recognizing a degraded state, not a reasoning error per se.
Incomplete output (IO) scales sharply from 4\% at easy to 34\% at hard, driven by Bridges (60\% at hard) and Galaxies (72\%), where the model fails to produce any complete answer.
Repeated reasoning (RR) peaks at medium (26\%) then declines at hard as ES rises, suggesting the model surrenders before it can enter repetitive cycles.
Constraint forgetting (CF) is rare under our strict definition (7\% at easy, 2\% at hard), and representation drift (RD) is driven almost entirely by Pattern (Appendix~\ref{app:per_puzzle_errors}).

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/llm_judge_v2/trace_verification_main_trio_normalized.png}
\caption{Prevalence of the seven main error categories by difficulty tier: aggregated across all five puzzle types (left, 250 traces per tier), and for Bridges (center) and Undead (right).
Bar labels show raw counts.
PC and STF increase with difficulty; ES and IO dominate at hard; RR peaks at medium then declines.
Four additional low-frequency categories are reported in Appendix~\ref{app:full_error_taxonomy}.}
\label{fig:error_trio}
\end{figure}

\paragraph{Intervention setup.}
The observational analysis identifies four error types that are plausibly causal rather than symptomatic: PC, STF, CF, and RR.
To test whether these patterns genuinely drive failure, we inject each error type into partial gold solution paths and measure downstream accuracy.
We evaluate DeepSeek-v3.2 on Bridges across three difficulty tiers (Easy/5$\times$5, Medium/7$\times$7, Hard/10$\times$10) with 100 puzzles per tier (300 per condition, 2,100 total API calls across 7 conditions), and replicate on Undead ($N{=}300$).
Each puzzle is presented with an unmodified partial gold path covering ${\sim}$15\% of the solution; intervention conditions apply a targeted modification before asking the model to continue.
All accuracy figures use 95\% Wilson score confidence intervals.

To generate intervention material, we expand the solver's solution paths into partial game trees by sampling legal-but-wrong moves at branching points and following wrong branches until a constraint violation terminates them.
Candidate prefixes that match any future gold state are discarded to prevent information leakage.
The four intervention types are: \textbf{RR}, $k{=}2$ wrong-path-then-backtrack cycles before the continuation point; \textbf{STF}, $k{=}3$ bridge cells flipped in the last intermediate grids while the action log is left intact; \textbf{CF}, one constraint violation (overcounting, crossing, or count modification) injected at the last step with no error signal; and \textbf{PC}, the gold prefix replaced with a wrong-path branch diverging at the first move, truncated before any obvious violation.
Full definitions and parameters are provided in Appendix~\ref{app:intervention_details}.

\paragraph{Intervention results.}
Figure~\ref{fig:intervention_forest} summarizes accuracy across all conditions for Bridges and Undead.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/interventions/intervention_forest_absolute.png}
\caption{Intervention effects on Bridges (circles, $N{=}300$) and Undead (squares, $N{=}300$).
Points show total accuracy with 95\% Wilson CIs; shaded bands mark the baseline.
PC and CF produce large, significant drops on both puzzles; STF reaches significance only on Undead; RR variants are indistinguishable from baseline.}
\label{fig:intervention_forest}
\end{figure}

PC ($-$20.8\,pp on Bridges, $-$11.3\,pp on Undead) and CF ($-$10.6\,pp, $-$11.3\,pp) produce large accuracy drops whose confidence intervals exclude the baseline on both puzzles.
STF occupies a middle tier: a borderline $-$7.8\,pp on Bridges (CI upper bound $+$0.3\,pp), strengthening to a significant $-$11.7\,pp on Undead where the model must track richer state.
RR is a null result on both puzzles; length-matched gold controls confirm that added context alone does not degrade performance.
We conclude that repeated reasoning in incorrect traces is a symptom of search, not a cause of failure.

\paragraph{Observational frequency is a poor proxy for causal impact.}
CF is among the least prevalent errors in the observational analysis (2--7\% of traces) yet produces one of the largest causal effects when injected.
The contrast with STF is informative: STF introduces a \emph{syntactic} inconsistency between grid and action log that the model can partially detect by cross-referencing the uncorrupted text, whereas CF produces an internally consistent state that violates puzzle rules, a \emph{semantic} error detectable only through active constraint verification.
The model largely lacks this capability, which explains why even rare constraint violations are so damaging.
Per-difficulty breakdowns are provided in Appendix~\ref{app:intervention_details}.


==> sections/diagnosis_v3.tex <==

\subsection{Diagnosing Failure Modes}
\label{sec:diagnosis}

To understand \emph{why} models fail on topology-heavy reasoning, we perform a systematic error analysis on full chains of thought, then design targeted interventions to test which failure modes genuinely degrade accuracy.
We focus on DeepSeek-v3.2, the strongest reasoning model among those in our evaluation that expose their complete chain of thought.

\textbf{Observational method.}
Following LLM-as-a-judge protocols~\citep{g_eval,prometheus}, we use GPT-5-mini to label each chain of thought according to an error taxonomy of eleven categories, of which seven are discussed in the main body (Table~\ref{tab:error_taxonomy_judge}) and the remainder in Appendix~\ref{app:full_error_taxonomy}.
We developed categories iteratively, first running a coarse labeling pass to surface prevalent behavioral patterns, then manually refining these into formal definitions.
The judge tags each trace with up to three labels and returns supporting excerpts for manual verification (prompt in Appendix~\ref{app:judge_prompt}).
In total we analyze 750 traces across 5 puzzle types and 3 difficulty tiers (50 per combination), excluding Loopy because even frontier models score near zero beyond the easy tier.

\input{sections/table_error_types_judge_v2}

\textbf{Observational results.}
Figure~\ref{fig:error_trio} summarizes error prevalence across difficulty tiers, both aggregated (left) and broken down for 2 representative puzzles: Bridges (center) and Undead (right).
Per-puzzle breakdowns for all five families appear in Appendix~\ref{app:per_puzzle_errors}.

Two error types scale sharply with difficulty.
The first, premature commitment (PC), triples from 13\% at easy to 40\% at hard, as committing to a wrong configuration early wastes the token budget on a dead-end branch from which the model struggles to recover.
The second, state-tracking failure (STF), shows the sharpest increases on Bridges and Undead, where rates climb from single digits at easy to 36\% at hard. On these puzzles, richer state, such as bridge counts and monster-type visibility constraints, overwhelms the model's internal bookkeeping.

The remaining high-frequency categories appear symptomatic rather than causal.
Explicit surrender and incomplete output both reflect an already-degraded reasoning state rather than being errors that initiate failure. Repeated reasoning peaks at medium difficulty but gives way to outright surrender at hard, suggesting the model abandons the problem before it can enter repetitive cycles (Figure~\ref{fig:error_trio}).
Representation drift is concentrated in Pattern and Galaxies and does not appear prominently in Bridges or Undead (Appendix~\ref{app:per_puzzle_errors}).
One category stands apart: constraint forgetting (CF) is rare and flat across difficulties (4--6\%), yet as the intervention experiments below will show, its low observational frequency hides a disproportionate causal impact.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/llm_judge_v2_updated/trace_verification_main_trio_normalized.png}
\caption{Prevalence of the seven main error categories by difficulty tier: aggregated across all five\protect\footnotemark puzzle types (left, 250 traces per tier), and for Bridges (center) and Undead (right). Bar labels show raw counts. PC and STF scale with difficulty; ES dominates at hard; IO is concentrated in Galaxies; RR peaks at medium then declines. Four additional low-frequency categories are reported in Appendix~\ref{app:full_error_taxonomy}.}
\label{fig:error_trio}
\end{figure}
\footnotetext{Loopy omitted because even frontier models score zero on medium and hard.}

\textbf{Intervention setup.}
To disentangle frequency from impact, we select four error types with distinct mechanistic profiles and test each via targeted injection. Premature commitment and repeated reasoning both waste the token budget, the former by pursuing dead-end branches and the latter by cycling through near-identical analyses that prevent forward progress.
Meanwhile, state-tracking failure and constraint forgetting both corrupt the model's representation of the puzzle, with state-tracking failure causing the model to lose track of the board state entirely, while constraint forgetting introduces rule violations that the model cannot detect, leaving it to build on a flawed foundation.
Of these four, PC and STF scale sharply with difficulty (PC triples from 13\% to 40\%, STF climbs from single digits to 36\% on Bridges and Undead), whereas CF and RR do not.
To test whether these mechanisms genuinely drive failure and whether observational frequency predicts causal impact, we inject each error type into partial gold solution paths and measure downstream accuracy.
We evaluate DeepSeek-v3.2 on Bridges across three difficulty tiers (Easy/5$\times$5, Medium/7$\times$7, Hard/10$\times$10) with 100 puzzles per tier (300 per condition, 2,100 total API calls across 7 conditions), and replicate on Undead ($N{=}300$).
Each puzzle is presented with an unmodified partial gold path covering ${\sim}$15\% of the solution; intervention conditions apply a targeted modification before asking the model to continue.
We verify in Appendix~\ref{app:baseline_calibration} that the unmodified baseline is competitive with DeepSeek-v3.2's standard evaluation accuracy, confirming that the gold prefix does not introduce a meaningful distribution shift.
All accuracy figures use 95\% Wilson score confidence intervals.

To generate intervention material, we expand the solver's solution paths into partial game trees by sampling legal-but-wrong moves at branching points and following wrong branches until a constraint violation terminates them.
Candidate prefixes that match any future gold state are discarded to prevent information leakage.
The four intervention types are: \textbf{RR}, $k{=}2$ wrong-path-then-backtrack cycles before the continuation point; \textbf{STF}, $k{=}3$ bridge cells flipped in the last intermediate grids while the action log is left intact; \textbf{CF}, one constraint violation (overcounting, crossing, or count modification) injected at the last step with no error signal; and \textbf{PC}, the gold prefix replaced with a wrong-path branch diverging at the first move, truncated before any obvious violation.
Full definitions and parameters are in Appendix~\ref{app:intervention_details}.

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\vspace{-1.2em}
\includegraphics[width=0.48\textwidth]{figures/interventions/intervention_forest_absolute.png}
\caption{Intervention effects on Bridges (circles, $N{=}300$) and Undead (squares, $N{=}300$).
Points show total accuracy with 95\% Wilson CIs; shaded bands mark the baseline.
PC and CF produce large, significant drops on both puzzles; STF reaches significance only on Undead; RR variants are indistinguishable from baseline.}
\label{fig:intervention_forest}
\vspace{-1em}
\end{wrapfigure}
\textbf{Intervention results.}
Figure~\ref{fig:intervention_forest} summarizes accuracy across all conditions for Bridges and Undead.
PC and CF produce the largest accuracy drops, with PC falling by 20.8\,pp on Bridges and 11.3\,pp on Undead, and CF by 10.6\,pp and 11.3\,pp respectively. In both cases, confidence intervals exclude the baseline.
STF has a weaker and less consistent effect, producing a borderline 7.8\,pp drop on Bridges but a significant 11.7\,pp drop on Undead, where the model must track richer state.
RR shows no effect on either puzzle. Length-matched gold controls confirm that added context alone does not degrade performance, so repeated reasoning in incorrect traces is a symptom of search, not a cause of failure.

\textbf{Observational frequency is a poor proxy for causal impact.}
CF is among the rarest errors in the observational analysis yet produces one of the largest causal effects when injected.
The contrast with STF helps explain why. STF introduces a \emph{syntactic} inconsistency between the grid and the action log, and the model can partially recover by cross-referencing the uncorrupted text.
CF, by contrast, produces an internally consistent state that violates puzzle rules, a \emph{semantic} error detectable only through active constraint verification.
The model largely lacks this capability, which explains why even rare constraint violations are so damaging.
Per-difficulty breakdowns are in Appendix~\ref{app:intervention_details}.


==> sections/error_analysis.tex <==
\section{Error Analysis}

\input{sections/table_error_types}

Outline/ pointers before writing 
\begin{enumerate}
\item We perform error analysis on full chains of thought to understand failure modes in topology-heavy reasoning.
\item We analyze DeepSeek-v3.2 because it is the most competent reasoning model we evaluate that provides full chains of thought.
\
\item Following prior ``LLM-as-a-judge'' evaluation protocols~\cite{g_eval,prometheus}, we use an LLM to label each chain of thought into a small set of error buckets. We develop these buckets iteratively: we first run a coarse pass over chains of thought with an LLM to identify prevalent behaviors (Summarized in Table), then manually curate and define the behaviors, and finally use the LLM as a judge to tag each example with up to three labels. The prompt is provided in Appendix~\ref{app:judge_prompt}. We also ask the judge to return the neighboring 15 characters around the error location to facilitate manual verification. Results are summarized in Fig.~\ref{fig:error_analysis}. and the manual verification revealed that amongst the ones tagged we found that there was [VALUE ] [METRIC] amongst the annotators.


\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/1.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/2.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/3.png}
\end{subfigure}
\caption{Error analysis from GPT-5 chain-of-thought evaluation.}
\label{fig:gpt5_cot_analysis}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/rlp_replay_n50/fig1_error_by_difficulty.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/rlp_replay_n50/fig1b_puzzles_affected.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/rlp_replay_n50/fig1c_puzzles_with_error.png}
\end{subfigure}
\caption{RLP replay error analysis ($n=50$).}
\label{fig:rlp_replay_error_analysis}
\end{figure}


\item To gain a fuller understanding of the reasoning behaviors exhibited by the LLM, we designed a novel error analysis protocol. Specifically, we modified the DeepSeek prompt to ensure the model produced structured outputs in the form \texttt{MOVE:} (e.g., \texttt{add bridges between islands 2 and 3}) and requested the model to print \texttt{INTERMEDIATE\_GRIDS} whenever it was unsure or when it began backtracking. We iterated on the prompt until we achieved [VALUE]\% compliance (semi-automated evaluation). Providing a worked example demonstrating the desired chain of thought substantially improved the degree to which the model generated interpretable structure in its reasoning process.

We then parsed the model's actions and intermediate grids from its chain of thought, and replayed the moves within the environment to reconstruct the game tree followed by the LLM. This enabled us to identify diverse behavioral patterns through analysis of the resulting graph structures (e.g., repeated reasoning (RR), premature commitment (PC)), feedback provided by the environment, discrepancies between the parsed current state and the environment's current state (state transition failure (STF), consistency failure (CF)), or early deviations from the final solution state (PC). The results from this analysis are reported in Fig.~\ref{fig:error_analysis}.


\paragraph{Results and validation.}
Summarize the main findings first (Fig.~\ref{fig:error_analysis}), then report: (i) the overall prevalence of each error type, and (ii) how error prevalence varies with puzzle difficulty.
Figure \ref{fig:gpt5_cot_analysis} shows the error analysis from GPT-5 chain-of-thought evaluation. Figure \ref{fig:rlp_replay_error_analysis} shows the RLP replay error analysis ($n=50$).

pointers

1. from llm as a judge cot analysis, we find some very interesting behavioral patterns, We see that there is more RR, STF  and explicit surrender for incorrect puzzles compared to the correct ones. Behaviors like CF, PC and RR are also present with the incorrect to correct ratio flipping when moving up in difficulty. Another interesting behaviour that's present often in hard puzzles is topic drift where the model starts to reason about random math problems during reasoning especially on hard puzzle where the model cannot solve the puzzle. This might be a observed effect of model failure rather any cause ffactor for model to fail. After manual analysis we also see that explicit surrender is often observed in the hard puzzles where model gives up after trying for more than 60k tokens ask requests the use of a python environment or tool. We hypothesize that these 2 are also symptomatic signs than causal reasons of failure. The other behavioural patterns like RR, STF, CF, PC and RD could be causal reasons for model failure because they could lead to context explosion (RR,PC), and context poisioning (STF, CF) which could lead to inefficient reasoning.

2. to further investigate the possible failure modes identified from llm as a judge error analysis, we look at the results from the rlp-replay based analysis to see if they corroborate. 

\paragraph{Replay validity.}
Add a small diagnostic table verifying that RLP-replay faithfully reconstructs model traces, e.g., (i) parsing success rate, (ii) fraction of replayed traces that reach the final grid state claimed by the model, and (iii) action legality rate.

\paragraph{Method comparison.}
Compare error detections from LLM-as-a-judge vs.\ RLP-replay (e.g., overlap / disagreement rates per error type), and include a few representative examples illustrating typical disagreement cases.

\paragraph{Link to interventions.}
Conclude by motivating the targeted interventions: each intervention perturbs the prompt/context in a way that selectively induces one failure signature from Table~\ref{tab:error_taxonomy}, while keeping a matched control condition fixed.




\end{enumerate}





==> sections/error_analysis_llm_judge.tex <==
\section{Error Analysis}
\label{sec:error_analysis}

To understand \emph{why} models fail on topology-heavy reasoning, we perform a systematic error analysis on full chains of thought.
We focus on DeepSeek-v3.2, the most competent reasoning model in our evaluation that exposes its complete chain of thought (14,000--42,000 tokens per puzzle).

\paragraph{Method.}
Following prior LLM-as-a-judge evaluation protocols~\citep{g_eval,prometheus}, we use an LLM to label each chain of thought with a small set of error categories.
We develop these categories iteratively: first, we run a coarse pass over chains of thought with an LLM to surface prevalent behavioral patterns; we then manually curate and define a taxonomy of failure modes (Table~\ref{tab:error_taxonomy_judge}); finally, we use the LLM as a judge to tag each chain of thought with up to three labels.
To facilitate manual verification, the judge is also asked to return the neighboring 15 characters around each identified error location.
The prompt is provided in Appendix~\ref{app:judge_prompt}.
%% TODO: Manual verification: the manual verification revealed that amongst the ones tagged we found that there was [VALUE] [METRIC] agreement amongst the annotators.

\input{sections/table_error_types_judge}

\paragraph{Results.}
Figure~\ref{fig:gpt5_cot_analysis} summarizes the prevalence of each error type, split by correctness (correct vs.\ incorrect final answer) and difficulty tier.
Several findings stand out.

\emph{Repeated reasoning and state-tracking failure dominate incorrect solutions.}
Across all three difficulty levels, repeated reasoning paths (RR) and state-tracking failure (STF) are substantially more frequent in incorrect chains of thought than in correct ones.
Approximately 60\% of incorrect puzzles exhibit repeated reasoning, cycling through near-duplicate analyses of the same subproblem without making forward progress.
STF affects roughly 60\% of incorrect solutions, indicating that the model frequently loses track of the prior moves it made, not reflecting the grid that it prints it has placed or which constraints remain unsatisfied.

\emph{Explicit surrender is pervasive on incorrect puzzles.}
Roughly 60\% of incorrect chains of thought across all difficulty levels end with the model explicitly giving up.
Manual inspection reveals that on hard puzzles this typically occurs after the model has generated more than 60,000 reasoning tokens and requests access to a Python environment or external tool.
We hypothesize that explicit surrender and topic drift (discussed below) are \emph{symptomatic} of failure rather than causal: the model gives up because it has already entered a degraded reasoning state, not the other way around.

\emph{Constraint forgetting and premature commitment shift with difficulty.}
Both CF and PC appear at all difficulty levels, but their incorrect-to-correct ratio changes as puzzles get harder.
On easy puzzles, CF and PC occur at comparable rates in correct and incorrect solutions.
On hard puzzles, the gap widens: incorrect solutions exhibit noticeably higher rates of both error types, consistent with the hypothesis that larger grids overwhelm the model's ability to track constraints and prune the search space.

\emph{Topic drift emerges on hard puzzles.}
A distinctive failure pattern on hard puzzles is \emph{topic drift}: the model abandons puzzle-specific reasoning and begins discussing unrelated mathematical problems (e.g., combinatorial proofs, graph theory exercises) mid-trace.
This behavior is nearly absent on easy and medium puzzles and appears to be triggered when the model cannot make progress, suggesting it is an artifact of failure rather than a contributing cause.

\emph{Representation drift correlates with correct solutions.}
Interestingly, representation drift i.e. where the model shifts between different ways of referring to grid elements is slightly more common in correct solutions than incorrect ones, particularly on easy puzzles.
This suggests that flexible re-representation may be an adaptive strategy rather than an error, though further investigation is needed.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/1.png}
    \caption{Easy}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/2.png}
    \caption{Medium}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figures/gpt5_cot_analysis/3.png}
    \caption{Hard}
\end{subfigure}
\caption{Error flags from LLM-as-a-judge analysis of DeepSeek-v3.2 chains of thought, split by correctness (blue = correct, orange = incorrect) and difficulty tier.
Repeated reasoning, state-tracking failure, and explicit surrender are the most discriminative error types between correct and incorrect solutions.}
\label{fig:gpt5_cot_analysis}
\end{figure}

\paragraph{Causal vs.\ symptomatic errors.}
We distinguish between error types that are plausibly \emph{causal} contributors to failure and those that are more likely \emph{symptomatic}.
Repeated reasoning (RR), state-tracking failure (STF), constraint forgetting (CF), and premature commitment (PC) can directly degrade solution quality: RR and PC lead to context explosion (the model wastes its token budget on unproductive or wrong-path exploration), while STF and CF lead to context poisoning (the model continues reasoning from an incorrect state or violated constraints, compounding errors downstream).
In contrast, explicit surrender, topic drift, and incomplete output tend to appear \emph{after} the model has already entered a degraded state, suggesting they are consequences rather than causes of failure.
This distinction motivates the targeted intervention experiments in Section~\ref{sec:interventions}, where we selectively induce each causal error type to measure its downstream impact on accuracy.


==> sections/error_analysis_llm_judge_v2.tex <==
\section{Error Analysis}
\label{sec:error_analysis}

To understand \emph{why} models fail on topology-heavy reasoning, we perform a systematic error analysis on full chains of thought.
We focus on DeepSeek-v3.2, the most competent reasoning model in our evaluation that exposes its complete chain of thought (14,000--42,000 tokens per puzzle).

\paragraph{Method.}
Following prior LLM-as-a-judge evaluation protocols~\citep{g_eval,prometheus}, we use GPT-5-mini to label each chain of thought with a small set of error categories.
We develop these categories iteratively: first, we run a coarse pass over chains of thought to surface prevalent behavioral patterns; we then manually curate and define a taxonomy of eleven failure modes (Table~\ref{tab:error_taxonomy_judge}); finally, the judge tags each chain of thought with up to three labels.
To facilitate manual verification, the judge also returns the neighboring 15 characters around each identified error location.
The prompt is provided in Appendix~\ref{app:judge_prompt}. (need to add human verified that the judgements are correct)
We analyze 300 traces in total: 5 puzzle types $\times$ 3 difficulty tiers $\times$ 20 traces each.

\input{sections/table_error_types_judge_v2}

\paragraph{Results.}
Figures~\ref{fig:error_aggregated} and~\ref{fig:error_per_puzzle} summarize the prevalence of each error type across difficulty tiers and puzzle types.
Several findings stand out.

\emph{Explicit surrender dominates and scales sharply with difficulty.}
ES is by far the most prevalent behavior, rising from 29\% of traces at easy to 54\% at medium and 66\% at hard (Figure~\ref{fig:error_aggregated}).
The scaling varies dramatically across puzzles: Galaxies reaches 75\% ES even at easy and 100\% at medium, while FlowFree climbs to 95\% at hard.
Bridges, the easiest puzzle in our suite, has near-zero ES across all difficulties.
We hypothesize that explicit surrender is \emph{symptomatic} of failure rather than causal: the model recognizes it has entered a degraded reasoning state and gives up, rather than the surrender itself causing the failure.

\emph{Premature commitment scales sharply with difficulty.}
PC more than triples from 11\% at easy to 19\% at medium and 35\% at hard.
When the search space is large, committing early to a wrong configuration is difficult to recover from: the model wastes its token budget exploring a dead-end branch, and the accumulated context makes it harder to backtrack effectively.
The per-puzzle breakdown reveals that FlowFree exhibits the strongest PC scaling (15\% $\rightarrow$ 30\% $\rightarrow$ 55\% from easy to hard), consistent with the path-routing nature of the puzzle where an early wrong path blocks later flows.
Pattern and Undead show sharp jumps to 45--50\% at hard.
Interestingly, Galaxies PC peaks at medium (35\%) then drops at hard (10\%), because the model surrenders before making meaningful commitments.

\emph{State-tracking failure jumps at hard.}
STF triples from 9\% at easy to 27\% at hard.
Larger grids overwhelm the model's ability to maintain an accurate internal representation of the board: the claimed state diverges from the cumulative effect of the model's own stated actions.
The jump is concentrated at the hard tier, where grid sizes are largest and the number of intermediate states the model must track is greatest.

\emph{Repeated reasoning peaks at medium then declines.}
RR rises from 24\% at easy to 29\% at medium, then drops to just 12\% at hard.
The per-puzzle data clarifies this pattern: FlowFree and Pattern both peak at 50\% RR at medium before declining, and Galaxies RR peaks at easy (50\%) then collapses to 5\% at hard.
Bridges has zero RR across all difficulties.
The decline at hard coincides with the sharp rise in ES meaning the model surrenders before it has the chance to enter repetitive reasoning cycles.

\emph{Constraint forgetting is rare.}
CF drops from 7\% at easy to 2\% at hard.
Under a strict definition that requires an explicit proposed action violating structural rules (overcounting, crossing, overwriting fixed cells), constraint violations are uncommon.
The model's failures are predominantly at the reasoning level---losing track of state, committing to wrong branches, or cycling---rather than at the level of violating the puzzle's structural rules.

\emph{Representation drift is highest at easy, driven by Pattern.}
RD is most prevalent at easy (34\%) and remains elevated at medium and hard (24--27\%).
This aggregate trend is driven almost entirely by Pattern, which exhibits extreme RD rates (70\% at easy, 65\% at medium, 50\% at hard), far above any other puzzle type.
Pattern puzzles require reasoning simultaneously about row and column constraints, which may naturally lead to shifting between different ways of referring to grid elements.
The elevated rate on easier puzzles suggests that flexible re-representation may be an adaptive strategy rather than a pure error.

\paragraph{Causal vs.\ symptomatic errors.}
We distinguish between error types that are plausibly \emph{causal} contributors to failure and those that are more likely \emph{symptomatic}. We hypothesize that repeated reasoning (RR) and premature commitment (PC) lead to \emph{context explosion}: the model wastes its finite token budget on unproductive or wrong-path exploration, leaving insufficient capacity to complete the puzzle.
State-tracking failure (STF) and constraint forgetting (CF) lead to \emph{context poisoning}: the model continues reasoning from an incorrect board state or violated constraints, compounding errors downstream.
In contrast, explicit surrender, topic drift, and incomplete output tend to appear \emph{after} the model has already entered a degraded state, suggesting they are consequences rather than root causes of failure.

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/llm_judge_v2/trace_verification_aggregated_normalized.png}
\caption{Error category prevalence by difficulty tier, aggregated across all five puzzle types (100 traces per tier).
Bar labels show raw counts.
ES dominates at all tiers and scales sharply with difficulty; PC and STF show pronounced increases at hard; RR peaks at medium then declines as ES rises.}
\label{fig:error_aggregated}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{figures/llm_judge_v2/trace_verification_per_puzzle_normalized.png}
\caption{Error category prevalence by puzzle type and difficulty tier (20 traces per cell).
Galaxies and FlowFree are dominated by ES even at lower difficulties.
FlowFree has the strongest PC scaling.
Pattern exhibits elevated RR and extreme RD across all tiers.
Bridges has the lowest overall error rates.}
\label{fig:error_per_puzzle}
\end{figure}


==> sections/error_analysis_llm_judge_v2_per_puzzle.tex <==
\section{Per-Puzzle Error Analysis}
\label{app:per_puzzle_errors}

This appendix provides a detailed breakdown of the LLM-as-judge error analysis (Section~\ref{sec:error_analysis}) for each of the five puzzle types.
All numbers are out of 20 traces per difficulty tier (easy / medium / hard).

\paragraph{Bridges.}
Bridges has the lowest overall error rates, consistent with its status as the most accurately solved puzzle type.
RR is entirely absent across all three difficulty tiers (0/20 at every level).
Errors concentrate at the hard tier: STF appears in 6/20 hard traces (30\%), PC in 3/20 (15\%), and RD in 4/20 (20\%).
At easy and medium, almost no causal errors are flagged---STF appears in just 1/20 at each tier, and CF, PC, and RR are all at zero or near-zero.
ES is also minimal (0/20 at easy and medium, 1/20 at hard), indicating that the model typically completes its reasoning attempt on this puzzle.
The most common flag at easy is OTH (5/20), suggesting behaviors that do not fit the standard taxonomy.

\paragraph{FlowFree.}
FlowFree exhibits the strongest PC scaling of any puzzle type: 3/20 at easy (15\%), 6/20 at medium (30\%), and 11/20 at hard (55\%).
This is consistent with the path-routing nature of the puzzle, where committing to a wrong flow path early blocks other flows and is difficult to recover from.
RR peaks at medium (10/20, 50\%) then declines at hard (6/20, 30\%), mirroring the aggregate pattern and coinciding with the sharp rise in ES (5/20 at easy, 15/20 at medium, 19/20 at hard---95\% at hard).
STF is modest (1/20 at easy and medium, 4/20 at hard).
HV is elevated at medium (8/20, 40\%), suggesting the model frequently claims false validation on medium-difficulty flow puzzles.
RD is nearly absent across all tiers.

\paragraph{Galaxies.}
Galaxies is the most difficult puzzle type for DeepSeek-v3.2, with extreme ES rates: 15/20 at easy (75\%), 20/20 at medium (100\%), and 18/20 at hard (90\%).
The model struggles with this puzzle even at the easiest tier.
RR peaks at easy (10/20, 50\%)---the model attempts repeated approaches before giving up---then declines to 6/20 at medium and just 1/20 at hard as ES takes over.
PC peaks at medium (7/20, 35\%) then drops at hard (2/20, 10\%), because the model surrenders too early to make meaningful commitments.
STF is flat across difficulties (3/20 at each tier, 15\%).
RD is elevated at easy (10/20, 50\%), possibly reflecting the model's attempts to find an effective representation for galaxy symmetry constraints.
IO spikes at hard (17/20, 85\%), indicating the model frequently fails to produce a complete answer on hard Galaxies puzzles.

\paragraph{Pattern.}
Pattern shows the most distinctive error profile.
RR is elevated across all tiers (7/20 at easy, 10/20 at medium, 3/20 at hard), with the peak at medium (50\%) being the highest RR rate of any puzzle.
RD is extreme: 14/20 at easy (70\%), 13/20 at medium (65\%), and 10/20 at hard (50\%)---far above any other puzzle type.
Pattern puzzles require simultaneous reasoning about row and column constraints, which may naturally lead to shifting between different ways of referring to grid elements.
CF is also highest for Pattern at easy (5/20, 25\%), though it drops to near zero at medium and hard.
PC shows a pronounced jump at hard (9/20, 45\%), compared to 3/20 at both easy and medium (15\%).
STF follows a similar pattern, jumping from 1/20 at easy and medium to 5/20 at hard (25\%).
ES scales with difficulty (5/20, 12/20, 15/20) but remains lower than Galaxies or FlowFree.

\paragraph{Undead.}
Undead shows the highest STF rate at hard of any puzzle type: 9/20 (45\%), with a steady increase from 3/20 at easy (15\%) through 5/20 at medium (25\%).
PC also jumps sharply at hard (10/20, 50\%), compared to 4/20 at easy and 2/20 at medium.
RR is moderate and relatively flat (2--3/20 across difficulties).
RD is elevated at easy and medium (9/20 each, 45\%) but drops at hard (4/20, 20\% -- possibly replaced by ES at 13/20, 65\%).
HV appears primarily at medium and hard (4/20 and 3/20).
ES scales from 4/20 at easy (20\%) to 7/20 at medium (35\%) and 13/20 at hard (65\%), following the aggregate trend.


==> sections/formats.tex <==
% --- Input Format Intervention ---

\subsubsection{Input Format Intervention}
\label{subsec:format-intervention}

Since the two-dimensional structure of puzzles tokenizes unfavorably (see Figure~\ref{fig:rugged_boundaries}), we hypothesize that weak performance may be driven by tokenization issues rather than reasoning limitations per se. We therefore re-evaluate \emph{identical} puzzle instances under four input encodings.

\noindent
\textbf{ASCII:} plain-text grid producing ragged token boundaries under standard tokenizers. \\
\textbf{IntFormat:} cells are encoded as numeric values, separated by commas, yielding more uniform, cell-aligned tokenization. \\
\textbf{IntFormat-JSON:} IntFormat wrapped in a two-dimensional JSON list, easily parseable by models with strong JSON understanding (used, e.g., in ARC-AGI~\citep{chollet2025arcagi2}). \\
\textbf{ASCII+image:} ASCII grid accompanied by a programmatically rendered image of the p

% \begin{itemize}[leftmargin=*,itemsep=2pt]
%     \item \textbf{ASCII:} plain-text grid producing ragged token boundaries under standard tokenizers.
%     \item \textbf{IntFormat:} cells are encoded as numeric values, separated by commas, yielding more uniform, cell-aligned tokenization.
%     \item \textbf{IntFormat-JSON:} IntFormat wrapped in a two dimensional JSON list. Easily parseable by models with strong JSON understanding. (used e.g. in ARC-AGI~\citep{chollet2025arcagi2})
%     \item \textbf{ASCII+image:} ASCII grid accompanied by a programmatically rendered image of the puzzle.
% \end{itemize}


Many tokens straddle cell boundaries, merging parts of adjacent cells into single tokens and destroying the two-dimensional board structure at the token level.
IntFormat and IntFormat-JSON use more tokens overall but preserve cell-boundary alignment, keeping the board's spatial structure intact in the token stream.


%On hard Undead and Pattern puzzles, gpt-5-mini routinely approaches or exceeds the 100k-token budget, which is why we do a rerun with a 200k-token budget for these puzzles. (link figure in tokens_bydifficulty_appendix.tex)


% \begin{figure}[t]
% \centering
% \includegraphics[width=\textwidth]{figures/formats/rugged_boundaries_bridges.png}
% \caption{Tokenization of a Bridges puzzle. ASCII (left) produces ragged boundaries that straddle grid cells; IntFormat (right) yields uniform, cell-aligned tokens preserving board structure.}
% \label{fig:rugged_boundaries}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[height=2.2cm]{figures/formats/rugged_boundaries_bridges_ascii.png}
    \hspace{0.3cm}
    \includegraphics[height=2.2cm]{figures/formats/rugged_boundaries_bridges_intformat_csv.png}
    \hspace{0.3cm}
    \includegraphics[height=2.2cm]{figures/formats/rugged_boundaries_bridges_intformat_json.png}
    \caption{Tokenization of a Bridges puzzle with gpt-5-mini's tokenizer (via tiktoken - CITE). ASCII (left) produces ragged boundaries that straddle grid cells; IntFormat (right) yields uniform, cell-aligned tokens preserving board structure.}
    \label{fig:rugged_boundaries}
\end{figure}



\paragraph{Results.}
Table~\ref{tab:format_comparison} summarizes accuracy across all four input formats.



% \begin{table}[ht]
% \centering
% \caption{Accuracy (\%) by input format across puzzle types. $\Delta$ rows show paired change relative to Plain ASCII (only models evaluated in both formats contribute).}
% \label{tab:format_comparison}
% \begin{tabular}{lrrrrrr}
% \toprule
% Format & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% Plain ASCII & 14.1 & 24.2 & 0.1 & 3.1 & 17.4 & 24.1 \\
% \midrule
% $\Delta$ With Image & +2.7 & +3.3 & +0.0 & -0.3 & -4.9 & \cellcolor[HTML]{FADBD8} -5.6 \\
% $\Delta$ Int-Format & \cellcolor[HTML]{D5F5E3} +5.1 & \cellcolor[HTML]{D5F5E3} +14.1 & +1.0 & +8.4 & -4.5 & -4.1 \\
% $\Delta$ Int-Format JSON & +2.7 & +10.9 & \cellcolor[HTML]{D5F5E3} +5.1 & \cellcolor[HTML]{D5F5E3} +8.8 & \cellcolor[HTML]{FADBD8} -8.6 & -3.1 \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\caption{Per-model accuracy (\%) by input format. Each model's $\Delta$ rows show change relative to its own Plain ASCII baseline.}
\label{tab:tab:format_comparison}
\begin{tabular}{lrrrrrr}
\toprule
Model / Format & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
\midrule
\textbf{DeepSeek V3.2} & 26.7 & 63.3 & 0.0 & 1.3 & 44.0 & 50.0 \\
\quad $\Delta$ With Image & -- & -- & -- & -- & -- & -- \\
\quad $\Delta$ Int-Format & \cellcolor[HTML]{D5F5E3} +6.7 & \cellcolor[HTML]{D5F5E3} +27.3 & +2.0 & \cellcolor[HTML]{D5F5E3} +28.0 & -26.0 & \cellcolor[HTML]{FADBD8} -7.3 \\
\quad $\Delta$ Int-Format JSON & +3.3 & +24.7 & \cellcolor[HTML]{D5F5E3} +9.0 & +23.3 & \cellcolor[HTML]{FADBD8} -36.7 & -6.0 \\
\midrule
\textbf{GPT-5 Mini} & 30.0 & 68.7 & 0.0 & 19.3 & 73.0 & 75.2 \\
\quad $\Delta$ With Image & +0.7 & -0.7 & +0.0 & -0.7 & -5.2 & -17.8 \\
\quad $\Delta$ Int-Format & \cellcolor[HTML]{D5F5E3} +8.0 & +12.0 & +0.0 & +15.3 & \cellcolor[HTML]{FADBD8} -7.9 & \cellcolor[HTML]{FADBD8} -21.8 \\
\quad $\Delta$ Int-Format JSON & +4.7 & \cellcolor[HTML]{D5F5E3} +15.3 & \cellcolor[HTML]{D5F5E3} +16.0 & \cellcolor[HTML]{D5F5E3} +17.3 & -7.0 & -12.5 \\
\midrule
\textbf{Gemini 3 Flash} & 42.7 & 58.0 & 0.0 & 5.3 & 29.3 & 66.0 \\
\quad $\Delta$ With Image & +4.7 & +7.3 & +0.0 & +0.0 & -4.7 & \cellcolor[HTML]{D5F5E3} +6.7 \\
\quad $\Delta$ Int-Format & +8.0 & +37.3 & +0.0 & \cellcolor[HTML]{D5F5E3} +32.0 & -6.0 & +3.3 \\
\quad $\Delta$ Int-Format JSON & \cellcolor[HTML]{D5F5E3} +10.0 & \cellcolor[HTML]{D5F5E3} +38.7 & \cellcolor[HTML]{D5F5E3} +8.0 & +29.3 & \cellcolor[HTML]{FADBD8} -25.3 & +4.7 \\
\bottomrule
\end{tabular}
\end{table}

IntFormat and IntFormat-JSON yield substantial accuracy improvements over ASCII, particularly on Bridges (+14.1\% and +10.9\%) and Galaxies (+8.4\% and +8.8\%). However, they also cause accuracy drops on Undead (-4.5\% and -8.6\%) and Pattern (-4.1\% and -3.1\%), suggesting that better tokenization alignment helps on average but interacts with puzzle-specific reasoning demands. Adding an image alongside ASCII does not consistently help, with marginal improvements on FlowFree and Bridges but declines on Undead and Pattern, indicating that current vision-language models struggle to integrate visual grid information with textual reasoning for structured constraint tasks.




==> sections/interventions.tex <==

\section{Interventions}

In error analysis section, we found strong presence of certain error types in the chain of thought of deepseekv3.2-reasoner. To validate if these errors are the causal link for these errors occurring we conduct intervention experiments for 5 of the most frequent error types. To enable these intervention experiment, we expand the solution path from the solver solver in the rlp codebase, by sampling k invalid moves at each branching point and then going down m steps in an invalid path. This effectively gives us a partial game-trees which can then be reused to construct interventions. Our interventions are peformed by prefilling the model with intervention specific prompt P-i and intervention specific part from the Int-data-i which is obtained after performing  transformation T operation on the partial game tree G. We define the different error buckets, and interventions below. 



REPEATED REASONING PATHS
The model repeatedly explores equivalent or previously rejected reasoning paths (e.g., DFS/BFS-style traversal or Hamiltonian path simulation) without pruning, abstraction, or convergence. The reasoning cycles through near-duplicate analyses without making forward progress.

Intervention : We sample 1 wrong dead end path , and add that to context, multiple times till step t<N where N is total number of steps. Then as the model to solve from t. t, is a correct grid state.  
Control: We give solution path till t and then ask the model to solve from there. Ideally we will keep t < N/2 or N/4 so that it's not trivial. 

add dead end paths to context and ask it to solve. 
just for 2 puzzles and compare with control !! 

STATE TRACKING FAILURE
The model fails to consistently track evolving state across steps (e.g., positions, filled cells, connections), leading to contradictions, impossible transitions, or mutually inconsistent assumptions within the same solution attempt.

Intervention: Probabilistically flip non-problem grid symbols in an intermediate grid in the solver path till t. Only at t, or at i<t steps. We will keep the actions same. This would mean that grid state tracking failed because of auto-regressive decoding. 
Control: We give solution path till t and then ask the model to solve from there. Ideally we will keep t < N/2 or N/4 so that it's not trivial. 

CONSTRAINT FORGETTING
The model forgets, misapplies, or violates explicit problem constraints (e.g., immutable endpoints, adjacency rules, uniqueness requirements). This includes overwriting fixed elements or breaking stated game rules.

Intervention: Probabilistically flip problem grid symbols in an intermediate grid in the solver path till t. Only at t, or at some i<t steps. We will keep the actions consistent with correct trace, because the model doesn't usually make this mistake on it's own. 
Control: We give solution path till t and then ask the model to solve from there. Ideally we will keep t < N/2 or N/4 so that it's not trivial. 



PREMATURE COMMITMENT
The model commits early to a specific configuration or hypothesis and continues refining it despite accumulating contradictions, failing to backtrack or reconsider foundational assumptions.

Intervention: Give model a wrong path at t=0 and then ask it to continue solving from there.
Control: Give the correct grid at t=0 and continue to solve

EXPLICIT SURRENDER
The model explicitly acknowledges inability to complete the task by requesting permission to use a programmatic solver, asking for more time, requesting relaxed constraints, or otherwise stating it cannot proceed as required.

This is a result of model not being able to solve, and not a cause for failure? -- correlation to token count? Does it happen when the model realizes it's going to hit a conext limit ?

INCOMPLETE OUTPUT
The model fails to produce a complete, valid final answer. Examples include partially filled solutions, placeholder symbols (e.g., dots or blanks), returning the original unsolved puzzle, or providing only a fragment of the required output.

This is a result of model not being able to solve, and not a cause for failure. 

UNJUSTIFIED ELIMINATION
The model prematurely eliminates valid possibilities, paths, or configurations without sufficient justification, leading to dead ends or incorrect conclusions about solvability.

This is very hard to design an intervention for. 

HALLUCINATED VALIDATION
The model asserts that a solution is correct, complete, or satisfies all constraints without proper verification, or despite the presence of contradictions, invalid configurations, or failed verification signals.

This is very hard to design an intervention for. 


REPRESENTATION DRIFT
The model’s internal representation of the problem changes over time (e.g., reinterpretation of symbols, coordinates, endpoints, or rules), resulting in inconsistent reasoning across different parts of the trace.

Intervention: give solution path with alternating int-format and co-ordinate representations 
Control: Compare with co-ordinate and int-format representations.

TOPIC DRIFT
The model shifts focus away from the original problem domain and does not answer the original task.

Not too many, ignore, Also this might be a result of model failing catastrophically and not a cause for model failure. 

OTHER
Use only if the observed failure does not reasonably fit any category above. If used, briefly describe the additional failure mode and why it is distinct.




Refined 


\section{Intervention Experiments} (Refined)

\subsection{Methodology}
In our error analysis, we identified a strong prevalence of specific error types in the chain-of-thought (CoT) traces of \texttt{deepseekv3.2-reasoner} (Figure \ref{fig:error_counts}). To determine if these error phenotypes are causal drivers of failure rather than merely symptomatic, we conduct intervention experiments targeting the five most frequent error categories.

To enable these experiments, we expand the solution path from the standard solver in the RLP codebase. At each branching point, we sample $k$ invalid moves and traverse $m$ steps down an invalid path. This yields a set of partial game trees, denoted as $G$, which serve as the substrate for constructing interventions.

Our general intervention protocol involves prefilling the model's context window with a manipulated partial solution. For a puzzle state at step $t$ (where $t < N$, the total solution steps), we construct a prompt consisting of a problem description $P$ and a partial reasoning trace $T_{\text{intervention}}$. We compare the model's success rate against a \textbf{Control} setup, where the model is provided with a correct, unmodified partial solution up to step $t$. To ensure non-triviality, we generally target split points where $t \approx N/4$ or $N/2$.

\subsection{Error-Specific Interventions}

\paragraph{1. REPEATED\_REASONING\_PATHS}
\textit{Definition:} The model explores equivalent or previously rejected reasoning paths without pruning, often cycling through near-duplicate analyses.
\textit{Hypothesis:} The presence of circular or redundant reasoning in the context acts as a "cognitive trap" (priming effect) that actively degrades solvability, distinct from the performance loss caused by increased context length (distraction).

\begin{itemize}
    \item \textbf{Methodology:} We employ a 3 pronged experimental design to isolate the causal mechanism:
    \begin{enumerate}
        \item \textbf{Clean Control ($C_{\text{clean}}$):} The model is provided with a concise, optimal solution path up to a valid intermediate state $S_{\text{valid}}$.
        \item \textbf{Noise Control ($C_{\text{noise}}$):} To control for context window saturation, we append $L$ tokens of "distractor" reasoning to the history of $S_{\text{valid}}$. These tokens are drawn from a \textit{different} puzzle instance (Out-of-Distribution logic) to simulate the cognitive load of reading irrelevant traces without introducing specific misleading cues for the current grid.
        \item \textbf{Intervention ($I_\text{loop}$):} We inject a short "reasoning loop" of length $L$ into the history repeated k times. For state $S_\text{valid}$, we simulate a sequence where the model attempts a plausible but invalid move $M_\text{bad}$, hits a contradiction, backtracks, and immediately re-attempts $M_\text{bad}$ (e.g., $S_\text{valid} \to S_\text{bad} \to S_\text{valid} \to S_\text{bad}$). backtracks to valid-- follows right steps to St. then ask model to solve from st
    \end{enumerate}
    \item \textbf{Causal Test:} We measure solvability rates $P(\text{solve})$.
    \begin{itemize}
        \item If $P(I_\text{loop}) \approx P(C_\text{noise}) < P(C_\text{clean})$, the failure is likely due to \textit{context length limitations}.
        \item If $P(I_\text{loop}) \ll P(C_\text{noise})$, the failure is caused by the \textit{specific content} of the loop, where the model is primed to repeat the error despite negative feedback in the context.
    \end{itemize}
\end{itemize}

\paragraph{2. STATE\_TRACKING\_FAILURE}
\textit{Definition:} The model fails to track evolving states (e.g., filled cells, connections), leading to contradictions between the board state and the reasoning text.
\begin{itemize}
    \item \textbf{Intervention:} We inject a \textit{Representation Mismatch}. Given a valid reasoning trace up to step $t$, we probabilistically flip non-fixed grid symbols (the player's moves) in the ASCII grid representation of step $t$, while keeping the natural language action history ("I moved X to Y") unchanged. Here the flipped states should still be valid states. 
    \item \textbf{Hypothesis:} This forces the model to resolve the conflict between its action history and its "visual input" current grid. Failure indicates an over-reliance on the potentially hallucinated visual state.
\end{itemize}

\paragraph{3. CONSTRAINT\_FORGETTING}
\textit{Definition:} The model violates explicit problem constraints (e.g., overwriting immutable endpoints).
\begin{itemize}
    \item \textbf{Intervention:}  We provide a history up to step $t$ where the previous move $a_{t-1}$ violated a constraint (e.g., overwrote a fixed digit), but the provided grid state updates as if the move were legal, without any error flags in the text.
    \item \textbf{Hypothesis:} This tests if the model actively verifies legality against the ground-truth rules at every step, or if it assumes the provided context is correct by definition.
\end{itemize}

\paragraph{4. PREMATURE\_COMMITMENT}
\textit{Definition:} The model persists with a specific hypothesis despite accumulating contradictions, failing to backtrack to the root cause.
\begin{itemize}
    \item \textbf{Intervention:} We provide a deep partial solution (depth $m$) derived from an incorrect move at $t=0$. We append reasoning text expressing high confidence in this flawed branch (e.g., "The configuration for the first three paths is solid...").
    \item \textbf{Hypothesis:} This evaluates the model's "Sunk Cost" resistance—can it abandon a significant amount of pre-filled context when it realizes the puzzle is unsolvable from the current state?
\end{itemize}

\paragraph{5. REPRESENTATION\_DRIFT}
\textit{Definition:} The model's internal representation (symbols, coordinates) becomes inconsistent.
\begin{itemize}
    \item \textbf{Intervention:} We provide a solution path where the format of the grid or the coordinate system alternates between steps (e.g., switching between integer-encoding and character-encoding, or 0-indexed vs 1-indexed coordinates) within the history.
    \item \textbf{Hypothesis:} This increases the cognitive load of translation. A failure here indicates the model lacks a robust, abstract internal world model and relies on pattern matching the immediate syntax.
\end{itemize}

\subsection{Excluded Categories}
We exclude \textbf{EXPLICIT\_SURRENDER} and \textbf{INCOMPLETE\_OUTPUT} from intervention experiments, as these are typically terminal symptoms of failure (or context window limits) rather than causal mechanisms. \textbf{UNJUSTIFIED\_ELIMINATION} and \textbf{HALLUCINATED\_VALIDATION} are excluded due to the difficulty of programmatically generating realistic interventions that mimic these subtle reasoning flaws.

\subsection{Results}


==> sections/interventions_n50.tex <==
\section{Intervention Experiments}
\label{sec:interventions}

The error analysis in Section~\ref{sec:error_analysis} identified four plausibly causal error types: repeated reasoning (RR), state-tracking failure (STF), constraint forgetting (CF), and premature commitment (PC).
To test whether these behavioral patterns are genuine causal drivers of failure rather than mere correlates of difficulty, we design targeted interventions that selectively inject each error type into the model's reasoning context and measure the downstream impact on accuracy.

\paragraph{Setup.}
We evaluate DeepSeek-v3.2 on Bridges puzzles across three difficulty tiers (Easy/5$\times$5, Medium/7$\times$7, Hard/10$\times$10), with 50 puzzles per tier and 150 per condition (1,200 total API calls across 8 conditions).
Each puzzle is presented with a \emph{partial gold solution path} covering approximately 15\% of the total solution steps.
For the baseline condition, this path is unmodified; for each intervention condition, a targeted modification is applied before the model is asked to ``solve the puzzle, starting from the last state.''
All accuracy figures are reported with 95\% Wilson score confidence intervals.

\paragraph{Game tree construction.}
To generate the raw material for interventions, we expand the puzzle solver's solution paths into partial game trees by sampling alternative moves at branching points---primarily legal-but-wrong moves such as a different bridge count on the same island pair or a connection to a different island---and following the resulting wrong paths for up to five steps until a constraint violation or engine rejection terminates the branch.
This yields both correct and incorrect branch prefixes that can be composed into intervention-specific traces.
To prevent information leakage, all candidate intervention prefixes are checked against future gold solution states; if a candidate intervention state matches any future gold state, it is discarded and a new prefix is sampled, ensuring no leakage occurs within each condition.

\paragraph{Intervention definitions.}
We define four intervention types, each targeting one causal error category from Table~\ref{tab:error_taxonomy_judge}, plus a gold control:

\begin{itemize}
\item \textbf{Repeated Reasoning (RR).}
A wrong-path exploration followed by a backtrack is injected into the trace $k{=}2$ times before the continuation point.
The model sees: gold path $\to$ wrong path $\to$ backtrack $\to$ wrong path $\to$ backtrack $\to$ correct state.
We test two variants: \emph{RR Samepoint}, where the two wrong paths diverge from the same branching state (maximizing diversity), and \emph{RR Standard}, where the same wrong path is repeated.
Both are leakage-free.

\item \textbf{RR Gold Control.}
A length-matched control that replaces the wrong-path segments with repetitions of the correct state.
If the effect of RR comes purely from increased context length rather than the specific content of the wrong paths, this control should produce the same effect.

\item \textbf{RR Rand Control.}
A length-matched control that replaces the wrong-path segments with randomly sampled incorrect moves from the game tree, unrelated to the continuation point.
Unlike the gold control, this inserts irrelevant wrong-path content, testing whether any extended context---not just correct-state repetition---affects performance.

\item \textbf{State-Tracking Failure (STF).}
We corrupt intermediate grid states while leaving the natural-language action history unchanged, creating a mismatch between the visual grid and the textual action log.
We report STF $k{=}3$, which independently flips a bridge cell in each of the last three grids; additional variants (fewer corruptions, cascading propagation that preserves inter-step consistency) produced similar non-significant effects and are discussed in the results.

\item \textbf{Constraint Forgetting (CF).}
A constraint violation is injected at the last step, uniformly sampled from three subtypes: overcounting an island's bridge capacity, introducing an illegal bridge crossing, or modifying an island's required count.
The grid updates as if the illegal move were legal, with no error signal in the text.
This tests whether the model actively verifies legality against the puzzle rules or simply trusts the provided context.

\item \textbf{Premature Commitment (PC).}
The gold path prefix is replaced entirely with a wrong-path branch that diverges from the gold solution at the very first move and extends to half the depth of the longest available incorrect branch, with no backtrack signal.
Because the path is truncated well before the dead-end, the final state does not exhibit an obvious constraint violation, making the corruption hard to detect.
This tests the model's sunk-cost resistance: can it detect and recover from an inherited wrong configuration?
\end{itemize}

\paragraph{Results.}
Table~\ref{tab:intervention_results} summarizes accuracy across all conditions.

\begin{table}[t]
\centering
\small
\caption{Intervention results on Bridges (accuracy \%, 50 puzzles per difficulty).
95\% Wilson CIs shown for the Total column.
$^\dagger$CI does not contain the baseline point estimate.}
\label{tab:intervention_results}
\begin{tabular}{lccccc}
\toprule
\textbf{Condition} & \textbf{Easy} & \textbf{Medium} & \textbf{Hard} & \textbf{Total} & $\boldsymbol{\Delta}$ \\
\midrule
Baseline            & 92.0 & 86.0 & 24.0 & 67.3 {\scriptsize [59.5, 74.3]} & -- \\
\midrule
RR Gold Ctrl        & 94.0 & 80.0 & 36.0 & 70.0 {\scriptsize [62.2, 76.8]} & $+$2.7 \\
RR Rand Ctrl        & 94.0 & 80.0 & 24.0 & 66.0 {\scriptsize [58.1, 73.1]} & $-$1.3 \\
RR Samepoint        & 94.0 & 74.0 & 30.0 & 66.0 {\scriptsize [58.1, 73.1]} & $-$1.3 \\
RR Standard         & 90.0 & 76.0 & 30.0 & 65.3 {\scriptsize [57.4, 72.5]} & $-$2.0 \\
\midrule
STF $k{=}3$         & 86.0 & 76.0 & 24.0 & 62.0 {\scriptsize [54.0, 69.4]} & $-$5.3 \\
\midrule
PC Half             & 94.0 & 58.0 &  8.0 & 53.3 {\scriptsize [45.4, 61.1]} & $-$14.0$^\dagger$ \\
CF Random           & 80.0 & 64.0 & 14.0 & 52.7 {\scriptsize [44.7, 60.5]} & $-$14.7$^\dagger$ \\
\bottomrule
\end{tabular}
\end{table}

\emph{The model cannot recover from early commitment errors.}
PC produces a $-$14.0pp accuracy drop, with its confidence interval excluding the baseline point estimate.
Because the wrong path diverges from the very first move, PC tests whether the model can detect an inherited wrong trajectory and course-correct; the results show it largely cannot.
We note that PC replaces the entire gold prefix---a more severe perturbation than the last-step modifications used by STF and CF---but the per-difficulty breakdown shows Easy accuracy is unaffected, suggesting the effect is not driven by the sheer amount of corruption.

\emph{Constraint forgetting is rare in natural traces but catastrophic when injected.}
CF ($-$14.7pp) is the largest causal effect in our study, and its CI upper bound falls below the baseline point estimate.
Yet in the error analysis (Section~\ref{sec:error_analysis}), CF is among the \emph{least} prevalent error types (2--7\% of traces), revealing that correlational error frequency is a poor proxy for causal impact.
For structural violations (overcounting, crossing), the action text describes the illegal move and the grid updates consistently with it---the corruption is internally consistent and detectable only through semantic verification of puzzle constraints (e.g., ``does this island already have its full bridge count?'').
Once an illegal state is introduced, the model trusts and builds on it.

\emph{State-tracking failure produces a mild, non-significant effect.}
STF $k{=}3$ ($-$5.3pp) does not reach significance; we tested seven variants spanning independent and cascading corruption across one to three grids, all producing similar effects ($-$2 to $-$5pp) with broadly overlapping confidence intervals.
The contrast with CF is informative: STF introduces a \emph{syntactic} inconsistency between two representations of the same state (the corrupted grid versus the intact action log), whereas CF produces an \emph{internally consistent} state that violates puzzle rules---a \emph{semantic} error detectable only by active constraint checking.
The model's partial resilience to STF suggests it can leverage the uncorrupted action history to detect grid corruption, while the much larger CF effect ($-$15pp vs.\ $-$5pp) indicates that verifying move legality against puzzle constraints is substantially harder.
In natural model traces, both STF and some CF instances may originate from stochastic errors during autoregressive grid reproduction.
Our interventions confirm that grid corruption alone trends negative but does not, by itself, account for the large accuracy gaps observed in the error analysis.

\emph{Repeated reasoning is a null result.}
Neither RR Samepoint ($-$1.3pp) nor RR Standard ($-$2.0pp) differs meaningfully from the baseline; all confidence intervals overlap broadly.
The gold control ($+$2.7pp) and random control ($-$1.3pp) also show no significant effect, confirming that neither the specific wrong-path content nor the mere extension of context length causally affects performance.
We conclude that the repeated reasoning patterns observed in incorrect chains of thought (Section~\ref{sec:error_analysis}) are more likely a \emph{symptom} of the model searching for a solution rather than a causal contributor to failure.

\paragraph{Summary.}
The intervention experiments reveal a two-tier separation among the error types identified in our error analysis.
Premature commitment ($-$14pp) and constraint forgetting ($-$15pp) produce strong causal effects whose confidence intervals exclude the baseline point estimate.
State-tracking failure produces a consistent but mild penalty ($-$5pp) that does not reach significance even in the most severe variant tested, and repeated reasoning shows no effect.
The STF--CF contrast suggests a mechanistic distinction: STF corruption is a syntactic inconsistency between the grid and the action log that the model can partially detect, whereas CF corruption is internally consistent but semantically illegal, requiring active constraint verification that the model struggles to perform.
A cross-puzzle replication on Undead confirms that CF and RR findings generalize, while PC effects are attenuated at lower baselines (Appendix~\ref{app:undead_interventions}).


==> sections/introduction.tex <==

\section{Introduction}
\label{sec:introduction}

Large language models (LLMs) and vision-language models have achieved strong performance on many algebraic~\cite{cobbe2021gsm8k}, symbolic, and textual reasoning benchmarks, yet their behavior on tasks that require visual thinking remains brittle. By visual thinking, we mean reasoning over a structured two-dimensional state where correct solutions depend on both local actions and global constraints---e.g., preserving connectivity, enforcing region consistency, or avoiding topological violations across a grid. Recent evaluations suggest that grid- and graph-structured settings remain among the most challenging categories for contemporary models, even when those models succeed on purely textual reasoning tasks~\cite{ren2025vgrp,long2025puzzleplex,chen2025enigmata}. 


A core difficulty in visual thinking is that the relevant constraints are often global and must be maintained through a sequence of partial states. Humans routinely solve such problems in logic puzzles that demand topological consistency—ensuring paths connect correctly, loops close without crossings, regions satisfy symmetry or partition constraints, and intermediate commitments remain compatible with future moves. Despite their suitability as stress tests for stateful spatial reasoning, topology-heavy puzzles are underrepresented in widely used benchmarks, which often emphasize short-horizon decisions, locally checkable rules, or formats that minimize the need to track evolving 2D structure~\cite{long2025puzzleplex,ren2025vgrp}. This leaves a gap in our ability to evaluate and diagnose whether modern models can robustly maintain global spatial invariants over multi-step problem solving.
To address this, we introduce TopoBench, a benchmark of six topology-focused puzzle families—Flow Free, Bridges, Galaxies, Undead, Pattern, and Loopy—chosen to span a range of visual load. We define visual load as the extent to which solving requires tracking and updating global spatial structure (e.g., connectivity, enclosure, crossings, symmetry-induced partitions) rather than applying predominantly local rules in isolation. TopoBench instances are constructed in difficulty tiers (easy/medium/hard) designed to progressively increase the burden of global constraint management. We evaluate a diverse set of open-source and closed-source models in both “open” and “closed” evaluation settings (depending on the task format and solver interface), enabling comparisons across model families and evaluation paradigms.


Our experiments show that topology-heavy visual reasoning remains difficult for current models. Even strong reasoning-oriented closed-source models that perform well on many text-centric tasks exhibit large performance drops on TopoBench’s hardest instances, leaving a substantial gap to human performance (e.g., models around 30--40\% versus a human baseline around 95\% on hard variants in our setting). These failures are not merely a function of puzzle size: performance degrades most sharply when the need for global state maintenance and consistent constraint propagation increases. In addition, we find that aggregate performance is highly sensitive to input representation. When the same underlying puzzle state is presented in representations that make the grid easier to parse and maintain (e.g., formats with more uniform tokenization and clearer structural cues), both open-source and closed-source models improve substantially relative to ASCII-like baselines. This sensitivity suggests that intermediate-state representation can be a first-order bottleneck for visual thinking.


However, benchmark scores alone do not explain why models fail. To move beyond accuracy, we conduct targeted failure analysis using two complementary approaches: (i) an environment-grounded replay analysis that reconstructs intermediate actions and states from model traces and compares them against solver-derived solution structures; and (ii) an LLM-assisted trace analysis that labels reasoning traces into interpretable error categories. Across both analyses, model failures concentrate around a small set of recurring breakdowns: premature commitment (committing early to a local configuration that later violates global constraints), state-tracking failure (losing track of the current grid state or earlier commitments), and constraint forgetting (dropping or misapplying previously established constraints). While other behaviors such as repeated reasoning appear frequently in traces, they do not consistently predict failure in our controlled tests, suggesting they may reflect benign search artifacts rather than a root cause.


Finally, we ask whether these failure modes are merely correlated with poor performance or are causal bottlenecks. We design intervention experiments that restart models from partial puzzle states derived from gold solution paths, while selectively modifying those partial states to target specific failure sources (e.g., adding premature commitment paths, state poisioning with missing constraints, or wrong tracked state). Across multiple puzzles and difficulty levels, interventions targeting premature commitment, state tracking failure, and constraint forgetting produce statistically significant changes in solve rates under controlled comparisons, supporting the conclusion that these are not incidental symptoms but key mechanisms limiting performance. (For interpretability and instrumentation, our most detailed mechanistic analyses operate in an ASCII setting where intermediate states can be reliably extracted; we additionally evaluate performance impacts of improved representations in the main benchmark results.)
In summary, TopoBench provides both a challenging evaluation suite for topology-heavy visual thinking and a diagnostic framework for understanding how and why models fail under high visual and state-tracking load. Our results highlight that representation choices, global state maintenance, and commitment timing are central obstacles for current models—suggesting concrete directions for future model and interface design.
Contributions.
	1. TopoBench, a benchmark of six topology-focused puzzle families stratified by visual load and difficulty.
	2. A broad evaluation of leading open-source and closed-source models, showing persistent gaps on high-load topology reasoning and strong representation sensitivity.
	3. Two complementary failure analyses identifying dominant mechanistic error modes---premature commitment, state-tracking failure, and constraint forgetting---and intervention experiments that causally validate these error modes as key bottlenecks for successful topology-heavy visual reasoning.

==> sections/introduction_outline_v2.tex <==
% Introduction Outline v2 — "diagnose → validate → treat" framing
% Target: ~1.5 pages (10-page workshop paper)

\section{Introduction}
\label{sec:introduction}

% === PARAGRAPH 1: Motivation + Gap ===
% - LLMs strong on algebraic/symbolic reasoning
% - Brittle on structured 2D reasoning requiring global constraint maintenance
%   (connectivity, loop closure, region symmetry, visibility propagation)
% - Existing puzzle benchmarks emphasize local rules, short horizons, or
%   single encodings — topology-heavy puzzles underrepresented
% - This leaves a gap: we cannot evaluate whether models maintain global
%   spatial invariants over multi-step solving
% we need to write about topological reasoning -- some definition of what it is

% === PARAGRAPH 2: Introduce TopoBench ===
% - TopoBench: 6 topology-focused puzzle families
%   (Flow Free, Bridges, Galaxies, Undead, Pattern, Loopy)
% - Span a range of topological phenomena: path connectivity, region
%   partitioning, degree constraints, visibility propagation, loop formation
% - 3 difficulty tiers (easy/medium/hard) scaling global constraint burden
% - Multiple input encodings (ASCII, IntFormat, IntFormat-JSON, ASCII+image)
% - 10 models evaluated (3 closed-source, 7 open-source), no code execution
% - All instances verified by puzzle-specific constraint checkers

% === PARAGRAPH 3: Baseline Results (slim — "how hard is this") ===
% - Even strong closed-source reasoning models struggle:
%   GPT-5-mini ~0.25 aggregate on hard, Gemini ~0.10 on hard
% - Open-source models near zero on medium and hard
% - Performance degrades most sharply when global state-maintenance
%   burden increases, not merely puzzle size
% - Galaxies and Loopy near-zero for all models at hard
% - Establishes that topology-heavy reasoning is a genuine open problem

% === PARAGRAPH 4: Diagnostic Pipeline — Error Analysis ===
% - Accuracy alone doesn't explain WHY models fail
% - We perform systematic error analysis on full chains of thought
%   (LLM-as-judge on DeepSeek-v3.2 traces, 300 traces)
% - Identify recurring failure modes:
%   premature commitment (PC), state-tracking failure (STF),
%   constraint forgetting (CF), repeated reasoning (RR)
% - Key observation: error frequency does not predict causal importance
%   (CF is rare but, as we show, devastating)

% === PARAGRAPH 5: Diagnostic Pipeline — Causal Validation ===
% - To separate causal bottlenecks from incidental correlates,
%   we design intervention experiments
% - Inject each error type into partial gold solution paths,
%   measure downstream accuracy impact
% - PC (-14pp) and CF (-15pp) are causal — CIs exclude baseline
% - RR is null; STF mild (-5pp, not significant)
% - Mechanistic insight: STF = syntactic inconsistency (model can
%   cross-check); CF = semantic violation (model cannot verify
%   constraint legality)

% === PARAGRAPH 6: Targeted Mitigations ===
% - Having identified WHAT breaks models, we ask: can we fix each one?
% - Three targeted mitigations, each addressing a diagnosed failure mode:
%   (a) Representation change (IntFormat/JSON) → mitigates parsing errors
%       and state-maintenance burden (STF/CF pathway);
%       large accuracy gains, explained by cell-aligned tokenization
%   (b) Externalized state → directly removes STF by maintaining
%       state externally so the model doesn't have to track it
%   (c) Few-shot worked examples with planning → addresses PC by
%       demonstrating initial constraint analysis before committing
% - All three show positive results, demonstrating that diagnosed
%   bottlenecks are actionable

% === PARAGRAPH 7: Contributions ===
% \paragraph{Contributions.}
% \begin{enumerate}
%   \item TopoBench, a benchmark of six topology-focused puzzle families
%         with three difficulty tiers, multiple encodings, and
%         puzzle-specific verifiers.
%   \item A diagnostic pipeline combining error taxonomy with causal
%         intervention experiments, identifying premature commitment and
%         constraint forgetting as key bottlenecks while ruling out
%         repeated reasoning.
%   \item Three targeted mitigations (representation change, externalized
%         state, few-shot planning) that each address a specific diagnosed
%         failure mode and produce measurable accuracy improvements.
% \end{enumerate}
%
% One-sentence roadmap:
% Section~\ref{sec:related_work} situates TopoBench in the literature;
% Section~\ref{sec:benchmark} describes the benchmark;
% Section~\ref{sec:experiments} reports baseline results;
% Section~\ref{sec:error_analysis} presents the error analysis;
% Section~\ref{sec:interventions} details causal validation; and
% Section~\ref{sec:mitigations} evaluates targeted mitigations.


==> sections/introduction_v2.tex <==

\section{Introduction}
\label{sec:introduction}

Large language models have achieved strong performance on algebraic~\citep{cobbe2021gsm8k,hendrycks2021math}, symbolic, and textual reasoning benchmarks, yet they remain brittle on tasks that require maintaining global spatial invariants through a sequence of partial states.
Topology-heavy puzzles, where correct solutions depend on path connectivity, loop closure, region symmetry, or visibility propagation across a two-dimensional grid, are a natural stress test for this capability.
Despite their suitability, such puzzles are underrepresented in widely used benchmarks, which tend to emphasize short-horizon decisions, locally checkable rules, or single input encodings~\citep{long2025puzzleplex,ren2025vgrp,giadikiaroglou2024puzzlesurvey}.
This leaves a gap in our ability to evaluate and diagnose whether current models can robustly track and update global spatial structure over multi-step problem solving.

We introduce TopoBench, a diagnostic benchmark of six topology-focused puzzle families: Flow Free, Bridges, Galaxies, Undead, Pattern, and Loopy, chosen to span a range of topological phenomena: path connectivity and non-crossing (Flow Free), degree constraints with global connectivity (Bridges), region partitioning under rotational symmetry (Galaxies), visibility propagation through mirrors (Undead), joint row--column constraint satisfaction (Pattern), and closed-loop formation (Loopy).
Instances are organized into three difficulty tiers (easy, medium, hard) that progressively increase the burden of global constraint management.
Each puzzle can be presented in multiple input encodings (ASCII, IntFormat, IntFormat-JSON, and ASCII+image), enabling controlled comparisons that hold the underlying problem fixed while varying only its surface representation.
We evaluate ten reasoning-oriented models---two closed-source (GPT-5-mini, Gemini-3-Flash) and seven open-source---under a pure-reasoning protocol with no external code execution, and verify all solutions with puzzle-specific constraint checkers.

Topology-heavy reasoning is difficult for all models we evaluate.
On the hard tier, GPT-5-mini achieves an aggregate accuracy of approximately 0.25 and Gemini-3-Flash approximately 0.10, while open-source models are near zero.
Even on easy puzzles, most open-source models score below 0.50, and certain puzzle families (Galaxies, Loopy) remain at or near zero for all models at hard difficulty.
Performance degrades most sharply when the need for global state maintenance increases, establishing that topology-heavy spatial reasoning remains a genuine open problem for current architectures.

Accuracy alone, however, does not explain \emph{why} models fail.
To move beyond aggregate scores, we build a diagnostic pipeline with two stages.
First, we perform systematic error analysis on 300 full chains of thought from DeepSeek-v3.2, using an LLM-as-judge protocol to label each trace with interpretable error categories.
Model failures concentrate around a small set of recurring breakdowns: \emph{premature commitment} (PC)---committing early to a local configuration that later violates global constraints; \emph{state-tracking failure} (STF)---losing track of the current grid state; \emph{constraint forgetting} (CF)---dropping or misapplying puzzle rules; and \emph{repeated reasoning} (RR)---cycling through near-duplicate analyses.
A key observation is that error frequency in traces does not predict causal importance: CF appears in only 2--7\% of traces yet, as we show next, produces the largest causal effect when injected.

Second, we design intervention experiments that inject each error type into partial gold solution paths and measure downstream accuracy changes.
Premature commitment ($-$14\,pp) and constraint forgetting ($-$15\,pp) produce strong causal effects whose confidence intervals exclude the baseline, confirming these are genuine bottlenecks rather than incidental correlates of difficulty.
Repeated reasoning shows no effect, indicating that the cycling patterns observed in incorrect traces are symptomatic of search rather than a root cause of failure.
State-tracking failure produces a consistent but mild penalty ($-$5\,pp) that does not reach significance.
The contrast between STF and CF reveals a mechanistic distinction: STF introduces a \emph{syntactic} inconsistency between the grid and the action log that the model can partially detect by cross-referencing, whereas CF produces an \emph{internally consistent} state that violates puzzle rules---a \emph{semantic} error detectable only through active constraint verification, which models struggle to perform.

Having identified what breaks models, we ask whether targeted mitigations can address each diagnosed bottleneck.
We evaluate two structural interventions that change the \emph{interface} the model reasons over.
First, switching from ASCII to structured representations (IntFormat, IntFormat-JSON) yields large accuracy improvements---for example, Gemini-3-Flash improves from 0.05 to 0.90 on hard Bridges---explained by cell-aligned tokenization that reduces the parsing and state-reconstruction burden underlying STF and CF failures.
Second, augmenting the reasoning interface with tool-based state management and constraint queries improves accuracy on Bridges ($+$12\,pp medium, $+$10\,pp hard) and eliminates board-validity errors entirely; an additive ablation reveals that constraint queryability---not state externalization alone---is the critical factor, independently confirming the primacy of CF over STF.
Both mitigations produce measurable accuracy improvements, demonstrating that the diagnosed bottlenecks are not only identifiable but actionable.
We also investigate prompt-level interventions (few-shot examples, planning instructions, recovery demonstrations) targeting PC, but find that none significantly improve hard-tier accuracy---the model's extended-thinking process appears to dominate over prompt-level strategy guidance (Appendix~\ref{app:prompt_interventions}).

\paragraph{Contributions.}
\begin{enumerate}
\item \textbf{TopoBench}, a benchmark of six topology-focused puzzle families with three difficulty tiers, multiple input encodings, and puzzle-specific verifiers, designed to stress-test global spatial reasoning.
\item A \textbf{diagnostic pipeline} combining an error taxonomy with causal intervention experiments that identifies premature commitment and constraint forgetting as key bottlenecks while ruling out repeated reasoning as a causal factor.
\item Two \textbf{structural mitigations}---representation change and tool-augmented reasoning---that each address a specific diagnosed failure mode and produce measurable accuracy gains, alongside a negative result showing that prompt-level interventions targeting premature commitment are ineffective for reasoning models.
\end{enumerate}

Section~\ref{sec:related_work} situates TopoBench in the literature.
Section~\ref{sec:benchmark} describes the benchmark design.
Section~\ref{sec:experiments} reports baseline results.
Sections~\ref{sec:error_analysis} and~\ref{sec:interventions} present the diagnostic pipeline, and Section~\ref{sec:mitigations} evaluates targeted mitigations.


==> sections/introduction_v3.tex <==

\section{Introduction}
\label{sec:introduction}

Large language models have achieved strong performance on algebraic~\citep{cobbe2021gsm8k,hendrycks2021math}, symbolic, and textual reasoning benchmarks, yet they remain brittle on tasks that require maintaining global spatial invariants through a sequence of partial states.
Topology-heavy puzzles, whose solutions depend on path and network connectivity, loop closure, region symmetry, or reflection across a two-dimensional grid, are a natural stress test for this capability but remain underrepresented in widely used benchmarks~\citep{long2025puzzleplex,ren2025vgrp,giadikiaroglou2024puzzlesurvey}.

We introduce \textbf{TopoBench}, a diagnostic benchmark of six topology-focused puzzle families spanning diverse topological phenomena, organized into three difficulty tiers and presented in multiple input encodings (ASCII, IntFormat, IntFormat-JSON, and ASCII+image).
We evaluate nine reasoning-oriented models, both closed-source (GPT-5-mini, Gemini-3-Flash) and open-weight, under a pure-reasoning protocol with no external code execution, verifying all solutions with puzzle-specific constraint checkers.
Even on easy puzzles most open-weight models score below 0.50; on the hard tier, the best closed-source model reaches only ${\sim}0.28$, and certain puzzle families remain at or near zero across the board.

Accuracy alone does not explain \emph{why} models fail.
We build a diagnostic pipeline that combines systematic error analysis of 300 chains of thought with causal intervention experiments that inject specific error types into partial gold solution paths.
The pipeline identifies premature commitment and constraint forgetting as genuine bottlenecks with strong causal effects on downstream accuracy, while ruling out other frequently observed patterns (such as repeated reasoning) as correlates of difficulty rather than causes.

We then evaluate structural mitigations that target the diagnosed failure modes.
Cell-aligned representations reduce the parsing burden that underlies state-tracking errors, and tool-augmented reasoning with constraint queries addresses constraint forgetting directly; both improve accuracy.
Prompt-level interventions, by contrast, prove ineffective for reasoning models (Appendix~\ref{app:prompt_interventions}).

\paragraph{Contributions.}
\begin{enumerate}[nosep]
\item \textbf{TopoBench}, a benchmark of six topology-focused puzzle families with three difficulty tiers, multiple input encodings, and puzzle-specific verifiers, designed to stress-test global spatial reasoning.
\item A \textbf{diagnostic pipeline} combining error taxonomy with causal intervention experiments that identifies premature commitment and constraint forgetting as key bottlenecks.
\item Two structural mitigations (representation change and tool-augmented reasoning) that address specific diagnosed failure modes and improve accuracy, alongside a negative result on prompt-level interventions.



\end{enumerate}



% new versions:

% Large language models have achieved strong performance on algebraic~\citep{cobbe2021gsm8k,hendrycks2021math}, symbolic, and textual reasoning benchmarks, yet they remain brittle on tasks that require maintaining global spatial invariants through a sequence of partial states.
% Topology-heavy puzzles, whose solutions depend on global spatial constraints such as connectivity, loop closure, and symmetry over a two-dimensional grid, are a natural stress test for this capability but remain underrepresented in widely used benchmarks~\citep{long2025puzzleplex,ren2025vgrp,giadikiaroglou2024puzzlesurvey}.

% We introduce \textbf{TopoBench}, a diagnostic benchmark of six topology-focused puzzle families spanning diverse global spatial constraints, organized into three difficulty tiers and paired with puzzle-specific verifiers.
% Across a suite of strong closed and open LLMs evaluated without external code execution, performance remains low: most open-weight models achieve below 50\% accuracy even on the easy tier; on the hard tier, the best closed model reaches only ${\sim}0.28$ accuracy, and some families remain near-unsolved.

% To understand failure modes, we build a diagnostic pipeline that combines systematic error analysis of 750 model solution traces using LLM as a judge to understand the prevalance of error types, and follow  with controlled intervention experiments that edit partial gold solution prefixes to instantiate specific error types, then measure how downstream accuracy changes when the model continues from that state.
% This pipeline identifies premature commitment and constraint forgetting as bottlenecks with strong effects on downstream accuracy, while showing that other frequent patterns (e.g., repeated reasoning) are more correlated with difficulty than causally driving failure.

% We then evaluate structural mitigations that target the diagnosed failure modes.
% Cell-aligned representations reduce parsing and state-tracking errors, and structured constraint querying improves constraint adherence; both improve accuracy, whereas prompt-level strategy guidance is largely ineffective for reasoning models.

% \paragraph{Contributions.}
% \begin{enumerate}[nosep]
% \item \textbf{TopoBench}, a benchmark of six topology-focused puzzle families with three difficulty tiers and puzzle-specific verifiers for evaluating global spatial reasoning.
% \item A \textbf{diagnostic pipeline} combining an error taxonomy with controlled interventions on partial gold solution prefixes that isolates premature commitment and constraint forgetting as key bottlenecks.
% \item Structural mitigations (cell-aligned representations and structured constraint querying) that improve accuracy, alongside a negative result on prompt-level interventions.
% \end{enumerate}


==> sections/introduction_v4.tex <==

\section{Introduction}
\label{sec:introduction}

Large language models have achieved strong performance on algebraic~\citep{cobbe2021gsm8k,hendrycks2021math}, symbolic, and textual reasoning benchmarks, yet they remain brittle on tasks that require maintaining global spatial invariants through a sequence of partial states.
Topology-heavy puzzles, whose solutions depend on global spatial constraints such as path connectivity, loop closure, and region symmetry over a two-dimensional grid, are a natural stress test for this capability but remain underrepresented in widely used benchmarks~\citep{long2025puzzleplex,ren2025vgrp,giadikiaroglou2024puzzlesurvey}.

We introduce \textbf{TopoBench}, a diagnostic benchmark of six topology-focused puzzle families spanning diverse global spatial constraints, organized into three difficulty tiers and paired with puzzle-specific verifiers.
We evaluate nine reasoning-oriented models, two closed-source and seven open-weight, under a pure-reasoning protocol with no external code execution.
Three frontier models (GPT-5-mini, Gemini-3-Flash, DeepSeek-v3.2) lead substantially, with GPT-5-mini averaging 0.66 on easy puzzles and 0.28 on hard, but the remaining six models, including 32B reasoning-capable models, average at most 0.07 on easy, a gap far larger than standard reasoning benchmarks would predict.
Two puzzle families resist all models: Loopy is near-zero across every model and difficulty tier, and Galaxies exceeds 0.16 only for GPT-5-mini.

Accuracy alone does not explain \emph{why} models fail.
We build a diagnostic pipeline that combines LLM-as-a-judge error analysis of 750 solution traces with controlled intervention experiments that edit partial gold solution prefixes to instantiate specific error types, then measure downstream accuracy when the model continues from the corrupted state.
Premature commitment and constraint forgetting emerge as genuine bottlenecks with strong causal effects on downstream accuracy.
The causal picture diverges from the observational one: constraint forgetting appears in only 2--7\% of traces yet produces one of the largest accuracy drops when injected (${\sim}$11\,pp on both Bridges and Undead), while repeated reasoning, among the most visible patterns in solution traces, is causally null.
Observational error frequency is a poor proxy for what actually drives failure.

We evaluate structural mitigations targeting the diagnosed bottlenecks.
Cell-aligned integer encodings reduce the parsing burden by aligning tokenization with cell boundaries, yielding gains on four of six puzzle families (up to $+$14\,pp on Bridges).
Tool-augmented reasoning with structured constraint queries raises hard-Bridges accuracy from 40\% to 50\% and eliminates board-validity failures entirely.
Ablations reveal that externalizing the board as a rendered ASCII grid actually \emph{degrades} accuracy by 14\,pp, whereas providing the same constraint information as pre-computed structured fields produces the largest single gain ($+$16\,pp).
The model possesses sufficient reasoning capacity for these puzzles; what it cannot do reliably is extract actionable constraint information from spatial representations.
Prompt-level interventions (11 conditions including worked examples and planning instructions) are ineffective for reasoning models, with longer prompts correlating with worse hard-tier performance (Appendix~\ref{app:prompt_interventions}).

\paragraph{Contributions.}
\begin{enumerate}[nosep]
\item \textbf{TopoBench}, a benchmark of six topology-focused puzzle families with three difficulty tiers and puzzle-specific verifiers, on which even frontier models solve fewer than a third of hard instances and two families remain near-unsolved.
\item A \textbf{diagnostic pipeline} combining LLM-as-a-judge error taxonomy with controlled interventions on gold solution prefixes, revealing that premature commitment and constraint forgetting are causal bottlenecks while observational error frequency is a poor proxy for causal impact.
\item Structural mitigations (cell-aligned encodings and structured constraint queries) that improve accuracy by addressing diagnosed failure modes, with ablations showing that spatial constraint extraction, not reasoning ability, is the primary bottleneck; and a negative result on prompt-level interventions.
\end{enumerate}


==> sections/methodology.tex <==
\section{TopoBench: The Benchmark}


organization of the section -- small paragraph



\subsection{Topology focused puzzles}
\subsubsection{Puzzle Selection}


\textbf{Visual Load Taxonomy}

\textbf{Puzzle Difficulty Tiers}



\subsection{Representation Formats}


\subsection{Evaluation Setup}

\subsection{Error Analysis and Interventions}

==> sections/relatedwork.tex <==

% ============================================
\section{Related Work}
\label{sec:related_work}
% ============================================

Topo-Bench is motivated by a growing literature on evaluating and improving neural reasoning, spanning general-purpose reasoning benchmarks, puzzle and grid evaluations, multimodal reasoning, and analyses of how surface form interacts with model computation. Classic mathematical reasoning suites such as GSM8K~\citep{cobbe2021gsm8k} and MATH~\citep{hendrycks2021math} emphasize multi-step symbolic manipulation, while broader benchmark collections such as ARC~\citep{chollet2025arcprize} and BIG-Bench Hard~\citep{suzgun2022bigbenchhard} target abstraction and difficult compositional tasks. Complementary to these, code-focused evaluations such as HumanEval~\citep{chen2021humaneval} and LiveBench~\citep{white2024livebench} assess program synthesis and practical coding competence. In contrast to benchmarks that primarily vary task domain, Topo-Bench holds the underlying problem instance fixed while systematically varying its \emph{representation} (ASCII, integer grids, JSON, and image+text), enabling controlled measurement of representation sensitivity.

Recent work has also improved performance on multi-step tasks via prompting and structured inference. Chain-of-thought prompting~\citep{wei2022cot} and Zero-shot CoT~\citep{kojima2022zeroshotcot} encourage explicit intermediate reasoning, while more explicit search-style frameworks such as Tree of Thoughts~\citep{yao2023tot} and Graph of Thoughts~\citep{besta2024got} expand the space of candidate solution trajectories. Sampling-based aggregation methods such as Self-Consistency~\citep{wang2023selfconsistency} further improve robustness through majority voting, and process-level supervision via reward modeling~\citep{lightman2023verify} suggests that step-wise feedback can outperform outcome-only training. Our state-corruption and ``frozen update'' manipulations complement these lines of work by directly stress-testing an implicit assumption shared by many CoT-style approaches: that intermediate states remain internally consistent throughout long reasoning traces.

Puzzle- and grid-based evaluation has emerged as a particularly useful lens on structured reasoning. A recent survey by \citet{giadikiaroglou2024puzzlesurvey} organizes puzzle solving with LLMs into a taxonomy and motivates controlled analyses across puzzle types. Benchmark efforts include Sudoku-Bench~\citep{sudokubench2025} for Latin-square variants, SATBench~\citep{satbench2025} for satisfiability, and CrossWordBench~\citep{leng2025crosswordbench} for language-heavy puzzle solving, as well as game-based settings such as chess~\citep{toshniwal2022chess,harang2025chessstate} and Sokoban~\citep{sokobench2026} that emphasize planning and state maintenance. Methodologically, GridPuzzle~\citep{tyagi2024gridpuzzle} pioneered fine-grained error taxonomies and automated annotation of reasoning chains, while VGRP-Bench~\citep{vgrpbench2025}, Enigmata~\citep{chen2025enigmata}, and KORGym~\citep{shi2025korgym} provide additional visual-grid and interactive evaluation settings. Topo-Bench is aligned with these efforts in using verifiable, structured tasks, but differs in its emphasis on \emph{multi-encoding control} and in isolating state maintenance as a failure mode independent of problem difficulty.

Finally, our analysis is informed by work showing that model behavior can be highly sensitive to tokenization and surface form. Prior studies demonstrate that digit tokenization and number representation influence arithmetic performance~\citep{singh2024tokenization,nogueira2021arithmetic}, and that format perturbations as small as a single character can cause large swings in outcomes~\citep{su2025singlechar}. We extend this perspective to topological puzzles by linking cell-boundary alignment in tokenization to downstream accuracy differences across encodings. More broadly, Topo-Bench relates to the literature on state tracking in language models, spanning procedural text tracking~\citep{rezaee2025statetracking} and dialogue state tracking~\citep{budzianowski2018multiwoz}, as well as evidence for emergent internal board representations in game-like settings such as Othello-GPT~\citep{li2023othello,nanda2023othello}. Planning-oriented benchmarks further highlight the importance of maintaining coherent long-horizon states~\citep{zheng2026pilot}. Our contribution is to provide a controlled, verifiable setting where representation choices and deliberate state perturbations can be studied in isolation, clarifying when failures arise from reasoning versus from brittle state maintenance.

==> sections/results.tex <==
\subsection{Main Results}
\label{subsec:main-results}

\subsection{Main Results}
\label{subsec:main-results}

Table~\ref{tab:accuracy_combined} shows verifier-checked accuracy across models and puzzle families. Three models—GPT-5 Mini, Gemini 3 Flash, and DeepSeek V3.2—form a clear frontier tier, substantially outperforming all others. However, even these models degrade sharply with difficulty, and none achieve reliable performance on the hard tier, indicating that the benchmark remains largely unsolved.

The remaining models cluster near zero accuracy, even on easy puzzles, creating a much larger performance gap than typically observed on standard reasoning benchmarks. This suggests that topology-heavy puzzles require capabilities not broadly present across current model classes.

Performance also varies strongly by puzzle family. While some families show gradual degradation with difficulty, others remain near-zero even for the strongest models, pointing to specific failure modes related to global topological constraints.

Overall, the results reveal a sharp capability boundary: a small frontier tier demonstrates partial competence, but robust topological reasoning remains out of reach for current models.






The gap between the top three and remaining models is substantially larger than what standard reasoning benchmarks would predict, suggesting that topology-heavy puzzle solving requires capabilities not yet present in most current models.
For context, these easy-tier puzzles are routine for experienced human solvers~\citep{estermann2024puzzles}.




\begin{table}[htbp]
\centering
\small
\caption{Accuracy by model and puzzle type across difficulties. Rows with all-zero accuracy are omitted.}
\label{tab:accuracy_combined}
\begin{tabular}{lrrrrrrr}
\toprule
Model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern & Avg \\
\midrule
\multicolumn{8}{l}{\textbf{Easy}} \\
\midrule
DeepSeek V3.2 & \cellcolor[HTML]{C3E8CD} 0.62 & \cellcolor[HTML]{79CEA7} 0.92 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFAF3} 0.04 & \cellcolor[HTML]{A4E2CA} 0.76 & \cellcolor[HTML]{9FDFC5} 0.78 & \cellcolor[HTML]{D6E5C0} 0.52 \\
Gemini 3 Flash & \cellcolor[HTML]{AFE7D2} 0.72 & \cellcolor[HTML]{89D5B4} 0.86 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFEECF} 0.16 & \cellcolor[HTML]{9FDFC5} 0.78 & \cellcolor[HTML]{7FD0AB} 0.90 & \cellcolor[HTML]{CDE6C7} 0.57 \\
GLM-4.7 Flash & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFEFE} 0.00 \\
GPT-5 Mini & \cellcolor[HTML]{BCE9D2} 0.66 & \cellcolor[HTML]{7FD0AB} 0.90 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{CBE7C8} 0.58 & \cellcolor[HTML]{84D3B0} 0.88 & \cellcolor[HTML]{79CEA7} 0.92 & \cellcolor[HTML]{BDE8D1} 0.66 \\
GPT OSS 20B & \cellcolor[HTML]{FFF6E7} 0.08 & \cellcolor[HTML]{FFECC9} 0.18 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFFAF1} 0.05 \\
Mercury & \cellcolor[HTML]{FFEFD2} 0.15 & \cellcolor[HTML]{FFEFD2} 0.15 & \cellcolor[HTML]{FFFFFF} -- & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFF8ED} 0.06 \\
OLMo 3.1 32B & \cellcolor[HTML]{FFE6B7} 0.24 & \cellcolor[HTML]{FFF6E7} 0.08 & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFF6E7} 0.08 & \cellcolor[HTML]{FFF7EA} 0.07 \\
Qwen3-32B & \cellcolor[HTML]{FFECC9} 0.18 & \cellcolor[HTML]{FFF8ED} 0.06 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFEECF} 0.16 & \cellcolor[HTML]{FFF7EA} 0.07 \\
\midrule
\multicolumn{8}{l}{\textbf{Medium}} \\
\midrule
DeepSeek V3.2 & \cellcolor[HTML]{FFECC9} 0.18 & \cellcolor[HTML]{94DABD} 0.82 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{E1E4B9} 0.46 & \cellcolor[HTML]{C0E8CF} 0.64 & \cellcolor[HTML]{F5E1AC} 0.35 \\
Gemini 3 Flash & \cellcolor[HTML]{D2E6C3} 0.54 & \cellcolor[HTML]{BCE9D2} 0.66 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFF4E1} 0.10 & \cellcolor[HTML]{9FDFC5} 0.78 & \cellcolor[HTML]{F6E1AB} 0.35 \\
GPT-5 Mini & \cellcolor[HTML]{FFE8BD} 0.22 & \cellcolor[HTML]{AFE7D2} 0.72 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{99DDC1} 0.80 & \cellcolor[HTML]{7FD0AB} 0.90 & \cellcolor[HTML]{E5E3B7} 0.44 \\
GPT OSS 20B & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFEFE} 0.00 \\
OLMo 3.1 32B & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFAF3} 0.04 & \cellcolor[HTML]{FFFEFD} 0.01 \\
\midrule
\multicolumn{8}{l}{\textbf{Hard}} \\
\midrule
DeepSeek V3.2 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFEECF} 0.16 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFF4E1} 0.10 & \cellcolor[HTML]{FFF6E7} 0.08 & \cellcolor[HTML]{FFF9EE} 0.06 \\
Gemini 3 Flash & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{FFE8BD} 0.22 & \cellcolor[HTML]{FFFFFF} -- & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFE0A6} 0.30 & \cellcolor[HTML]{FFF3DE} 0.11 \\
GPT-5 Mini & \cellcolor[HTML]{FFFCF9} 0.02 & \cellcolor[HTML]{E5E3B7} 0.44 & \cellcolor[HTML]{FFFFFF} -- & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{DAE5BE} 0.50 & \cellcolor[HTML]{E7E3B5} 0.43 & \cellcolor[HTML]{FFE2AC} 0.28 \\
OLMo 3.1 32B & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} -- & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFFFF} 0.00 & \cellcolor[HTML]{FFFAF3} 0.04 & \cellcolor[HTML]{FFFEFC} 0.01 \\
\bottomrule
\end{tabular}
\end{table}

==> sections/state_externalization.tex <==
% --- State Externalization Intervention ---

\subsection{Tool-Augmented State Externalization}
\label{subsec:state-externalization}

To directly target state-tracking failure, we replace one-shot answer generation with an iterative tool-call interface in which the model solves the puzzle through a sequence of actions while an external engine maintains the authoritative board state.
We evaluate DeepSeek-v3.2 on Bridges at medium ($7{\times}7$, $N{=}50$) and hard ($10{\times}10$, $N{=}50$) difficulty.
The model has access to five tools spanning two categories: \emph{state-mutation} tools (\texttt{make\_move}, which applies a bridge and rejects illegal moves; \texttt{render\_board}, which returns the current ASCII grid) and \emph{constraint-query} tools (\texttt{state\_summary}, which reports each island's remaining bridge capacity; \texttt{neighbors}, which enumerates legal moves with corridor clearance and joint capacity; \texttt{components}, which returns connected components and candidate cross-component links).
No tool solves the puzzle or suggests an optimal move; the model must still decide which bridges to place and in what order.

\paragraph{Results.}
The full tool suite improves accuracy by $+$12\,pp on medium (80\%~$\to$~92\%) and $+$10\,pp on hard (40\%~$\to$~50\%).
The most striking effect is on board validity: on hard puzzles, only 50\% of baseline outputs are structurally valid boards, whereas the tool-augmented interface achieves 100\% validity across both difficulty tiers, completely eliminating board-modification errors.
This confirms that invalid boards in the baseline are caused by state-tracking failures rather than fundamental reasoning limitations.
Token consumption also decreases---from 25,640 to 17,571 on hard (a 31\% reduction)---because the model no longer spends tokens re-rendering and verifying the grid state within its chain of thought.

\paragraph{Ablation: what drives the gains?}
To isolate which components are responsible for the accuracy improvement, we run an additive ablation on hard Bridges ($N{=}50$), starting from state-mutation tools only and progressively adding each constraint-query tool.
Table~\ref{tab:tool_ablation} reports the results.

\begin{table}[ht]
\centering
\caption{Additive tool ablation on hard Bridges ($N{=}50$). Each row adds one tool on top of the previous condition. State mutation alone degrades accuracy relative to baseline; constraint-query tools---especially degree bookkeeping---drive recovery and gains.}
\label{tab:tool_ablation}
\begin{tabular}{llrrr}
\toprule
Condition & Tools available & Accuracy & Board valid & Avg tokens \\
\midrule
Baseline (no tools) & --- & 40\% & 50\% & 25{,}640 \\
State mutation only & \texttt{make\_move}, \texttt{render\_board} & 26\% & 96\% & 28{,}308 \\
\, + degree bookkeeping & + \texttt{state\_summary} & 42\% & 100\% & 22{,}784 \\
\, + move enumeration & + \texttt{neighbors} & 44\% & 100\% & 19{,}570 \\
\, + connectivity analysis & + \texttt{components} & 48\% & 98\% & 18{,}030 \\
Full tool suite & + candidate links & 50\% & 100\% & 17{,}571 \\
\bottomrule
\end{tabular}
\end{table}

The ablation reveals a surprising pattern.
State mutation alone---which externalizes the board but provides no constraint information---\emph{degrades} hard accuracy by 14\,pp relative to the baseline (26\% vs.\ 40\%), despite raising board validity from 50\% to 96\%.
The model loses the ability to reason holistically over the full board in a single pass and instead enters multi-turn loops of trial, error, and backtracking, without sufficient information to guide its decisions.
The critical recovery comes from adding \texttt{state\_summary}, which provides pre-computed degree bookkeeping (remaining bridges per island, overflow detection, global satisfaction checks).
This single tool accounts for the largest gain in the ablation ($+$16\,pp, from 26\% to 42\%), recovering baseline-level accuracy while maintaining 100\% board validity.
Subsequent tools contribute diminishing marginal returns: move enumeration adds 2\,pp, connectivity analysis adds 4\,pp, and candidate cross-component links add 2\,pp.
Token consumption decreases monotonically as more tools are added, from 28{,}308 (state mutation only) to 17{,}571 (full suite), reflecting fewer wasted exploratory steps when the model receives richer per-step information.

\paragraph{Interpretation.}
The ablation converges with the causal intervention results from Section~\ref{sec:interventions}: the binding bottleneck is constraint computation, not state representation.
In the intervention experiments, constraint forgetting ($-$10.6\,pp) produces a larger causal effect than state-tracking failure ($-$7.8\,pp) on Bridges; the ablation independently confirms this ranking by showing that fixing state tracking alone is insufficient---and even counterproductive---while offloading constraint arithmetic is the factor that unlocks accuracy gains.
The ASCII grid is a lossless encoding of game state: all information needed to compute constraint satisfaction is present in principle.
However, extracting it requires spatial-algorithmic reasoning---scanning directions, counting bridge characters, computing degree gaps---that the model performs unreliably.
\texttt{state\_summary} converts this spatial extraction into pre-computed numeric fields (e.g., \texttt{remaining: 2}), shifting the task from perceptual parsing to algebraic comparison, which language models handle well.
State externalization is thus necessary (it eliminates board-validity errors) but insufficient (accuracy requires constraint queryability).


==> sections/state_externalization_v2.tex <==
% --- State Externalization Intervention (v2: Option D framing) ---

\subsubsection{Tool-Augmented Reasoning}
\label{subsec:state-externalization}

The formats intervention (Section~\ref{subsec:format-intervention}) showed that changing input representation produces large accuracy swings, suggesting that much of the model's difficulty lies in \emph{parsing} spatial state rather than \emph{reasoning} about constraints.
To test this hypothesis more directly, we replace one-shot answer generation with an iterative tool-call interface in which the model solves Bridges through a sequence of actions while an external engine maintains the authoritative board state and provides constraint information on demand.
We evaluate DeepSeek-v3.2 at medium ($7{\times}7$, $N{=}50$) and hard ($10{\times}10$, $N{=}50$) difficulty.

The model has access to up to five tools spanning two categories:
\begin{itemize}[nosep]
\item \emph{State-mutation tools}: \texttt{make\_move} (applies a bridge; rejects illegal moves) and \texttt{render\_board} (returns the current ASCII grid).
\item \emph{Constraint-query tools}: \texttt{state\_summary} (reports each island's required, current, and remaining bridge count, plus edge list and overflow detection); \texttt{neighbors} (enumerates legal moves per island with corridor clearance and joint capacity); \texttt{components} (returns connected components with isolation risk and candidate cross-component links).
\end{itemize}
No tool solves the puzzle or suggests an optimal move; the model must still decide which bridges to place and in what order.
The key design distinction is that state-mutation tools return information in the same spatial format as the original puzzle (an ASCII grid), while constraint-query tools return pre-computed structured data (JSON with numeric fields).

\paragraph{Results.}
The full tool suite improves accuracy by $+$12\,pp on medium (80\%~$\to$~92\%) and $+$10\,pp on hard (40\%~$\to$~50\%), while eliminating board-validity errors entirely (50\%~$\to$~100\% valid boards on hard).
Token consumption decreases from 25{,}640 to 17{,}571 on hard (31\% reduction), because the model no longer spends tokens re-rendering and verifying the grid state within its chain of thought.

\paragraph{Ablation: spatial vs.\ structured information.}
To understand what drives the accuracy gains, we run two ablation series on hard Bridges ($N{=}50$).
The first is an \emph{additive} ablation that starts from state-mutation tools only and progressively adds each constraint-query tool.
The second tests whether the spatial grid representation (\texttt{render\_board}) helps or hurts when structured alternatives are available.
Table~\ref{tab:tool_ablation} reports both.

\begin{table}[ht]
\centering
\caption{Tool ablation on hard Bridges ($N{=}50$).
\emph{Top}: additive ablation adding one tool per row.
\emph{Bottom}: grid removal variants testing whether \texttt{render\_board} helps when structured tools are available.
The grid is harmful with few tools and irrelevant with many.}
\label{tab:tool_ablation}
\begin{tabular}{llrrr}
\toprule
Condition & Tools available & Accuracy & Board valid & Avg tokens \\
\midrule
Baseline (no tools) & --- & 40\% & 50\% & 25{,}640 \\
\midrule
\multicolumn{5}{l}{\emph{Additive ablation}} \\
\, State mutation only & \texttt{make\_move}, \texttt{render\_board} & 26\% & 96\% & 28{,}308 \\
\, + degree bookkeeping & + \texttt{state\_summary} & 42\% & 100\% & 22{,}784 \\
\, + move enumeration & + \texttt{neighbors} & 44\% & 100\% & 19{,}570 \\
\, + connectivity & + \texttt{components} & 48\% & 98\% & 18{,}030 \\
\, Full suite & + candidate links & 50\% & 100\% & 17{,}571 \\
\midrule
\multicolumn{5}{l}{\emph{Grid removal}} \\
\, Structured only (2 tools) & \texttt{make\_move}, \texttt{state\_summary} & 46\% & 100\% & 27{,}301 \\
\, Structured only (4 tools) & all except \texttt{render\_board} & 50\% & 100\% & 22{,}294 \\
\bottomrule
\end{tabular}
\end{table}

The additive ablation reveals a surprising pattern.
State mutation alone---which externalizes the board but returns it in spatial format (ASCII)---\emph{degrades} accuracy by 14\,pp (26\% vs.\ 40\%), despite raising board validity from 50\% to 96\%.
Trace analysis shows the model enters multi-turn loops of trial, error, and backtracking: it calls \texttt{render\_board} 12.5 times per puzzle on average but cannot reliably extract constraint information from the rendered grid (e.g., counting bridges per island requires scanning four directions and decoding bridge characters).
Adding \texttt{state\_summary}---which provides the same constraint information as pre-computed numeric fields---produces the largest single gain ($+$16\,pp, from 26\% to 42\%).
Subsequent tools contribute diminishing returns: $+$2\,pp (neighbors), $+$4\,pp (connectivity), $+$2\,pp (candidate links).

The grid removal experiments sharpen the finding.
With only \texttt{state\_summary} available, physically removing \texttt{render\_board} from the tool list \emph{improves} accuracy by 4\,pp (42\%~$\to$~46\%).
When \texttt{render\_board} is available, the model calls it 8 times per puzzle on average regardless of prompt instructions to the contrary, and these spatial renderings appear to interfere with the algebraic reasoning that \texttt{state\_summary} enables.
With the full tool stack, removing \texttt{render\_board} has no effect (50\% either way): the richer constraint tools already provide sufficient structured data that the model barely relies on the grid (only 6 renders per puzzle), rendering it redundant.

\paragraph{Interpretation.}
The ablation results, combined with the format intervention in Section~\ref{subsec:format-intervention}, converge on a consistent finding: \textbf{the primary bottleneck is spatial constraint extraction, not reasoning ability.}
The model \emph{can} solve these puzzles---40\% baseline accuracy on hard Bridges demonstrates the underlying reasoning capability exists.
What it cannot do reliably is extract actionable constraint information from spatial representations.

Three independent lines of evidence support this:
\begin{enumerate}[nosep]
\item \emph{Format intervention}: switching from ASCII to IntFormat produces large accuracy gains on the same puzzles, by providing cell-aligned tokenization that reduces the spatial parsing burden.
\item \emph{Additive ablation}: \texttt{render\_board} (spatial state) degrades accuracy; \texttt{state\_summary} (structured constraints) recovers it. The tools provide the same underlying information in different formats---the structured format is what helps.
\item \emph{Grid removal}: when structured tools are available, removing the spatial grid either improves accuracy ($+$4\,pp with \texttt{state\_summary} alone) or has no effect (with the full tool stack). The spatial representation is never beneficial.
\end{enumerate}

The ASCII grid is a lossless encoding of game state: all information needed to verify constraint satisfaction is present in principle.
However, extracting it requires spatial-algorithmic reasoning---scanning directions from each island, decoding bridge characters (\texttt{-}, \texttt{=}, \texttt{|}, \texttt{"}), computing degree sums, checking corridor intersections---that the model performs unreliably.
\texttt{state\_summary} converts this spatial extraction into pre-computed numeric fields (e.g., \texttt{remaining:~2}), shifting the task from perceptual parsing to algebraic comparison.
The constraint-query tools do not merely \emph{reformat} existing information; they provide \emph{derived} quantities---remaining degree, joint capacity, connected components---that are absent from the grid and would require algorithmic computation to obtain.

State externalization is thus necessary (it eliminates board-validity errors) but insufficient (accuracy requires constraint queryability in structured form).
The parallel with the format intervention is direct: both results show that providing the same logical content in a more structured, less spatial encoding unlocks reasoning capability that is otherwise bottlenecked at the parsing stage.


==> sections/state_externalization_v3.tex <==
% --- State Externalization Intervention (v3: trimmed from v2) ---

\subsubsection{Tool-Augmented Reasoning}
\label{subsec:state-externalization}

To test this hypothesis more directly, we replace one-shot answer generation with an iterative tool-call interface in which the model solves Bridges through a sequence of actions while an external engine maintains the authoritative board state and provides constraint information on demand.
We evaluate DeepSeek-v3.2 at medium ($7{\times}7$, $N{=}50$) and hard ($10{\times}10$, $N{=}50$) difficulty.

The model has access to five tools in two categories.
\emph{State-mutation tools} (\texttt{make\_move}, \texttt{render\_board}) apply moves and return the board as an ASCII grid.
\emph{Constraint-query tools} (\texttt{state\_summary}, \texttt{neighbors}, \texttt{components}) return pre-computed structured data---remaining bridge counts, legal moves, connected components---as JSON (full specifications in Appendix~\ref{app:tool_augmented}).
No tool solves the puzzle or suggests an optimal move; the key design distinction is that state-mutation tools return spatial output while constraint-query tools return structured numeric fields.

\textbf{Results.}
The full tool suite improves accuracy by $+$12\,pp on medium (80\%~$\to$~92\%) and $+$10\,pp on hard (40\%~$\to$~50\%), while eliminating board-validity errors entirely (50\%~$\to$~100\% valid boards on hard).
Token consumption decreases from 25{,}640 to 17{,}571 on hard (31\% reduction), because the model no longer spends tokens re-rendering and verifying the grid state within its chain of thought.

\textbf{Ablation: spatial vs.\ structured information.}
To understand what drives the accuracy gains, we run two ablation series on hard Bridges ($N{=}50$).
The first is an \emph{additive} ablation that starts from state-mutation tools only and progressively adds each constraint-query tool.
The second tests whether the spatial grid representation (\texttt{render\_board}) helps or hurts when structured alternatives are available.
Table~\ref{tab:tool_ablation} reports both.

\begin{table}[ht]
\centering
\caption{Tool ablation on hard Bridges ($N{=}50$).
\emph{Top}: additive ablation adding one tool per row.
\emph{Bottom}: grid removal variants testing whether \texttt{render\_board} helps when structured tools are available.
The grid is harmful with few tools and irrelevant with many.}
\label{tab:tool_ablation}
\begin{tabular}{llrrr}
\toprule
Condition & Tools available & Accuracy & Board valid & Avg tokens \\
\midrule
Baseline (no tools) & --- & 40\% & 50\% & 25{,}640 \\
\midrule
\multicolumn{5}{l}{\emph{Additive ablation}} \\
\, State mutation only & \texttt{make\_move}, \texttt{render\_board} & 26\% & 96\% & 28{,}308 \\
\, + degree bookkeeping & + \texttt{state\_summary} & 42\% & 100\% & 22{,}784 \\
\, + move enumeration & + \texttt{neighbors} & 44\% & 100\% & 19{,}570 \\
\, + connectivity & + \texttt{components} & 48\% & 98\% & 18{,}030 \\
\, Full suite & + candidate links & 50\% & 100\% & 17{,}571 \\
\midrule
\multicolumn{5}{l}{\emph{Grid removal}} \\
\, Structured only (2 tools) & \texttt{make\_move}, \texttt{state\_summary} & 46\% & 100\% & 27{,}301 \\
\, Structured only (4 tools) & all except \texttt{render\_board} & 50\% & 100\% & 22{,}294 \\
\bottomrule
\end{tabular}
\end{table}

The additive ablation reveals a surprising pattern.
State mutation alone---which externalizes the board but returns it in spatial format (ASCII)---\emph{degrades} accuracy by 14\,pp (26\% vs.\ 40\%), despite raising board validity from 50\% to 96\%.
Trace analysis shows the model enters multi-turn loops of trial, error, and backtracking: it calls \texttt{render\_board} 12.5 times per puzzle on average but cannot reliably extract constraint information from the rendered grid.
Adding \texttt{state\_summary}---which provides the same constraint information as pre-computed numeric fields---produces the largest single gain ($+$16\,pp, from 26\% to 42\%).
Subsequent tools contribute diminishing returns: $+$2\,pp (neighbors), $+$4\,pp (connectivity), $+$2\,pp (candidate links).

The grid removal experiments sharpen the finding.
With only \texttt{state\_summary} available, physically removing \texttt{render\_board} from the tool list \emph{improves} accuracy by 4\,pp (42\%~$\to$~46\%).
When \texttt{render\_board} is available, the model calls it 8 times per puzzle on average regardless of prompt instructions to the contrary, and these spatial renderings appear to interfere with the algebraic reasoning that \texttt{state\_summary} enables.
With the full tool stack, removing \texttt{render\_board} has no effect (50\% either way): the richer constraint tools already provide sufficient structured data that the model barely relies on the grid, rendering it redundant.

\textbf{Interpretation.}
The ablation results converge with the format intervention (Section~\ref{subsec:format-intervention}) on a consistent finding: \textbf{the primary bottleneck is spatial constraint extraction, not reasoning ability.}
The model can solve these puzzles---40\% baseline accuracy on hard Bridges shows the underlying capability exists---but cannot reliably extract actionable constraints from spatial layouts.
The ASCII grid is a lossless encoding of game state, yet extracting constraint information from it requires spatial-algorithmic operations (scanning directions, decoding bridge characters, computing degree sums) that the model performs unreliably; \texttt{state\_summary} converts this into pre-computed numeric fields, shifting the task to algebraic comparison (see Appendix~\ref{app:tool_augmented} for a detailed discussion).
State externalization is thus necessary (it eliminates board-validity errors) but insufficient without structured constraint queryability.


==> sections/table_error_types.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.25}
\caption{Error taxonomy used for chain-of-thought error analysis. We provide (i) a human-readable definition, (ii) how each error is operationalized in simulator-grounded RLP-replay, and (iii) a targeted intervention designed to selectively elicit the failure mode (with a matched control).}
\label{tab:error_taxonomy}
\begin{tabular}{p{0.12\textwidth} p{0.30\textwidth} p{0.30\textwidth} p{0.28\textwidth}}
\toprule
\textbf{Error type} & \textbf{Definition (behavioral)} & \textbf{Detection in RLP-replay (operational)} & \textbf{Targeted intervention (w/ control)} \\
\midrule
\textbf{Repeated Reasoning (RR)} &
The model repeatedly explores equivalent or previously rejected reasoning paths (e.g., DFS/BFS-style traversal or Hamiltonian path simulation) without pruning, abstraction, or convergence. The reasoning cycles through near-duplicate analyses without making forward progress. &
The model re-executes long identical (or near-identical) action subsequences / state trajectories during replay, indicating cycling rather than progress (flagged when repetition exceeds a threshold). &
\textit{Intervention:} Sample one wrong dead-end path and add it to the context repeatedly up to step $t < N$ (where $N$ is the total number of steps), then ask the model to solve from $t$ (with a correct grid state at $t$). \textit{Control:} Provide the correct solution trace up to $t$ and ask the model to solve from there (choosing $t < N/2$ or $t < N/4$). \\
\midrule
\textbf{State-Tracking Failure (STF)} &
The model fails to consistently track evolving state across steps (e.g., positions, filled cells, connections), leading to contradictions, impossible transitions, or mutually inconsistent assumptions within the same solution attempt. &
The model's claimed intermediate grid disagrees with the simulator state obtained by replaying the parsed action sequence up to the same step. &
\textit{Intervention:} Probabilistically flip \emph{non-problem} grid symbols in an intermediate grid in the solver trace up to step $t$ (only at $t$ or at some $i<t$), while keeping the subsequent actions unchanged. \textit{Control:} Provide the correct trace up to $t$ and ask the model to solve from $t$ (choosing $t < N/2$ or $t < N/4$). \\
\midrule
\textbf{Constraint Forgetting (CF)} &
The model forgets, misapplies, or violates explicit problem constraints (e.g., immutable endpoints, adjacency rules, uniqueness requirements). This includes overwriting fixed elements or breaking stated game rules. &
The model attempts an action that the simulator rejects as illegal under the task rules (even if the model proceeds as if it were valid). &
\textit{Intervention:} Probabilistically flip \emph{problem} grid symbols in an intermediate grid in the solver trace up to step $t$ (only at $t$ or at some $i<t$), while keeping actions consistent with the correct trace. \textit{Control:} Provide the correct trace up to $t$ and ask the model to solve from $t$ (choosing $t < N/2$ or $t < N/4$). \\
\midrule
\textbf{Premature Commitment (PC)} &
The model commits early to a wrong branch, narrowing the search space and preventing recovery, even if the mistake is not immediately flagged by local constraints. &
In the replayed game tree, a branch begins with an early deviation that is inconsistent with the final solution trajectory (i.e., an unrecoverable wrong branch). &
\textit{Intervention:} Force an early commitment by injecting (or selecting) an incorrect but locally plausible early branch prefix, then ask the model to continue from the corresponding step $t$ and measure recovery. \textit{Control:} Continue from the matched step $t$ under the correct branch prefix. \\
\bottomrule
\end{tabular}
\end{table*}

==> sections/table_error_types_judge.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.25}
\caption{Error taxonomy for chain-of-thought analysis.
The first four error types (above the mid-rule) are plausibly \emph{causal} contributors to failure; the remaining types are more likely \emph{symptomatic} of an already-degraded reasoning state.
Each causal error type is paired with a targeted intervention designed to selectively elicit the failure mode (Section~\ref{sec:interventions}).}
\label{tab:error_taxonomy_judge}
\begin{tabular}{p{0.18\textwidth} p{0.52\textwidth} p{0.25\textwidth}}
\toprule
\textbf{Error type} & \textbf{Definition} & \textbf{Targeted intervention} \\
\midrule
\textbf{Repeated Reasoning (RR)} &
The model repeatedly explores equivalent or previously rejected reasoning paths without pruning or convergence, cycling through near-duplicate analyses without forward progress. &
Inject repeated dead-end paths into the context prefix up to step $t$; control provides the correct trace to $t$. \\
\midrule
\textbf{State-Tracking Failure (STF)} &
The model fails to consistently track evolving state across steps (e.g., placed bridges, remaining capacities), leading to contradictions or impossible transitions within the same solution attempt. &
Flip non-problem grid symbols in an intermediate state at step $t$; control provides the correct state at $t$. \\
\midrule
\textbf{Constraint Forgetting (CF)} &
The model forgets, misapplies, or violates explicit problem constraints (e.g., island capacities, bridge-crossing rules, adjacency requirements), including overwriting fixed elements. &
Flip problem grid symbols in an intermediate state at step $t$; control provides the correct state at $t$. \\
\midrule
\textbf{Premature Commitment (PC)} &
The model commits early to a wrong configuration, narrowing the search space and preventing recovery, even when the mistake is not immediately flagged by local constraints. &
Inject an incorrect but locally plausible branch prefix; control continues from the correct branch at $t$. \\
\midrule
\textbf{Explicit Surrender} &
The model explicitly gives up, often requesting access to a Python environment or external tool after exhausting its reasoning budget. &
--- \\
\midrule
\textbf{Topic Drift} &
The model abandons puzzle-specific reasoning and begins discussing unrelated problems (e.g., combinatorial proofs, graph theory exercises). &
--- \\
\midrule
\textbf{Representation Drift} &
The model shifts between different ways of referring to grid elements (e.g., coordinate systems, naming conventions) within the same chain of thought. &
--- \\
\bottomrule
\end{tabular}
\end{table*}


==> tables.tex <==





\begin{table}[htbp]
\caption{Accuracy on Easy Difficulty (Verifier)}
\label{tab:accuracy_easy}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
\midrule
deepseek-reasoner-error\_analysis & - & - & - & - & - & - \\
deepseek-v3.2 & 0.65 & 0.80 & - & 0.05 & 0.75 & 0.75 \\
deepseek-v3.2-intformat & 0.75 & 1.00 & - & 0.75 & 0.40 & 0.65 \\
gemini-3-flash-preview & 0.80 & 0.85 & 0.00 & 0.20 & 0.75 & 0.95 \\
gemini-3-flash-preview-intformat & 0.80 & 1.00 & 0.00 & 1.00 & 0.50 & 0.95 \\
gemini-3-flash-preview-intformat\_json & 0.85 & 1.00 & 0.20 & 1.00 & 0.30 & 0.95 \\
gemini-3-flash-preview-with-image & 0.85 & 0.90 & 0.00 & 0.00 & 0.65 & 0.90 \\
glm-4.7-flash & 0.05 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
glm-4.7-flash-intformat & 0.30 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
gpt-5-mini & 0.80 & 0.95 & 0.00 & 0.50 & 0.95 & 0.90 \\
gpt-5-mini-intformat & 0.80 & 1.00 & 0.00 & 0.90 & 0.95 & 0.90 \\
gpt-5-mini-intformat\_json & 0.85 & 1.00 & 0.30 & 0.90 & 0.80 & 0.90 \\
gpt-5-mini-with-image & 0.70 & 0.90 & 0.00 & 0.55 & 0.95 & 0.70 \\
gpt-oss-20b & 0.20 & 0.45 & - & 0.00 & 0.00 & 0.05 \\
gpt-oss-20b-intformat & 0.40 & 0.90 & - & 0.00 & 0.00 & 0.00 \\
llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
llama-4-maverick-17b-128e-instruct-intformat & 0.10 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
mercury & 0.15 & 0.15 & - & 0.00 & 0.00 & 0.00 \\
mercury-intformat & 0.25 & 0.65 & - & 0.00 & 0.00 & 0.00 \\
olmo-3.1-32b-think & 0.30 & 0.05 & - & 0.00 & 0.00 & 0.05 \\
olmo-3.1-32b-think-intformat & 0.50 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
qwen3-32b & 0.25 & 0.05 & - & 0.00 & 0.05 & 0.20 \\
qwen3-32b-intformat & 0.20 & 0.35 & - & 0.00 & 0.00 & 0.00 \\
qwen3-vl-235b-a22b-thinking & 0.45 & 0.65 & - & 0.00 & 0.35 & 0.25 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[htbp]
\caption{Accuracy on Hard Difficulty (Verifier)}
\label{tab:accuracy_hard}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
\midrule
gemini-3-flash-preview & 0.00 & 0.05 & 0.00 & 0.00 & 0.00 & 0.25 \\
gemini-3-flash-preview-intformat & 0.15 & 0.75 & 0.00 & 0.00 & 0.00 & 0.40 \\
gemini-3-flash-preview-intformat\_json & 0.20 & 0.90 & 0.00 & 0.00 & 0.00 & 0.40 \\
gemini-3-flash-preview-with-image & 0.00 & 0.25 & 0.00 & 0.00 & 0.00 & 0.25 \\
gpt-5-mini & 0.00 & 0.40 & 0.00 & 0.00 & 0.45 & 0.40 \\
gpt-5-mini-intformat & 0.05 & 0.55 & 0.00 & 0.00 & 0.15 & 0.00 \\
gpt-5-mini-intformat\_json & 0.05 & 0.75 & 0.00 & 0.00 & 0.25 & 0.20 \\
gpt-5-mini-with-image & 0.00 & 0.40 & 0.00 & 0.00 & 0.40 & 0.30 \\
\bottomrule
\end{tabular}}
\end{table}

% Commented out: duplicate hard accuracy table wrapped in \textit (invalid LaTeX)
% \textit{\begin{table}[htbp]
% \caption{Accuracy on Hard Difficulty (Verifier)}
% \label{tab:accuracy_hard}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% gemini-3-flash-preview & 0.00 & 0.05 & 0.00 & 0.00 & 0.00 & 0.25 \\
% gemini-3-flash-preview-intformat & 0.15 & 0.75 & 0.00 & 0.00 & 0.00 & 0.40 \\
% gemini-3-flash-preview-intformat\_json & 0.20 & 0.90 & 0.00 & 0.00 & 0.00 & 0.40 \\
% gemini-3-flash-preview-with-image & 0.00 & 0.25 & 0.00 & 0.00 & 0.00 & 0.25 \\
% gpt-5-mini & 0.00 & 0.40 & 0.00 & 0.00 & 0.45 & 0.40 \\
% gpt-5-mini-intformat & 0.05 & 0.55 & 0.00 & 0.00 & 0.15 & 0.00 \\
% gpt-5-mini-intformat\_json & 0.05 & 0.75 & 0.00 & 0.00 & 0.25 & 0.20 \\
% gpt-5-mini-with-image & 0.00 & 0.40 & 0.00 & 0.00 & 0.40 & 0.30 \\
% \bottomrule
% \end{tabular}
% \end{table}}



\begin{table}[htbp]
\caption{Board Extracted Rate - Hard Difficulty}
\label{tab:board_exists_hard}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
\midrule
deepseek-reasoner-error\_analysis & - & 1.00 & - & - & - & - \\
deepseek-v3.2 & 0.95 & 1.00 & - & 0.90 & 1.00 & 0.75 \\
deepseek-v3.2-intformat & 1.00 & 1.00 & - & 1.00 & 0.95 & 0.95 \\
gemini-3-flash-preview & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
gemini-3-flash-preview-intformat & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
gemini-3-flash-preview-intformat\_json & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
gemini-3-flash-preview-with-image & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
glm-4.7-flash & 0.30 & 0.40 & - & 0.35 & 0.00 & 0.40 \\
glm-4.7-flash-intformat & 0.30 & 0.30 & - & 0.30 & 0.30 & 0.65 \\
gpt-5-mini & 0.90 & 1.00 & 1.00 & 0.90 & 0.80 & 1.00 \\
gpt-5-mini-intformat & 0.85 & 1.00 & 0.75 & 0.90 & 0.65 & 0.95 \\
gpt-5-mini-intformat\_json & 0.75 & 1.00 & 0.70 & 0.50 & 0.55 & 0.75 \\
gpt-5-mini-with-image & 0.84 & 1.00 & 1.00 & 0.95 & 0.90 & 1.00 \\
gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
gpt-oss-20b-intformat & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
llama-4-maverick-17b-128e-instruct & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
mercury & 0.10 & 0.20 & - & 0.45 & 0.15 & 0.30 \\
mercury-intformat & 0.10 & 0.35 & - & 0.55 & 0.40 & 0.55 \\
olmo-3.1-32b-think & 1.00 & 1.00 & - & 0.60 & 1.00 & 1.00 \\
olmo-3.1-32b-think-intformat & 0.80 & 1.00 & - & 0.95 & 1.00 & 0.55 \\
qwen3-32b & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
qwen3-32b-intformat & 1.00 & 1.00 & - & 1.00 & 0.95 & 1.00 \\
qwen3-vl-235b-a22b-thinking & - & - & - & - & - & - \\
\bottomrule
\end{tabular}}
\end{table}

% OLD TABLES BELOW:
%
% % === EASY DIFFICULTY: ACCURACY ===
%
% \begin{table}[htbp]
% \caption{Accuracy on Easy Difficulty (Verifier)}
% \label{tab:accuracy_easy_old}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.65 & 0.80 & - & 0.05 & 0.75 & 0.75 \\
% gemini-3-flash-preview & 0.80 & 0.85 & - & 0.20 & 0.75 & 0.95 \\
% gemini-3-flash-preview-intformat & 0.80 & 1.00 & - & 1.00 & 0.50 & 0.95 \\
% gemini-3-flash-preview-with-image & 0.85 & 0.90 & - & 0.00 & 0.65 & 0.90 \\
% glm-4.7-flash & 0.05 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.30 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.80 & 0.95 & 0.00 & 0.50 & 0.95 & 0.90 \\
% gpt-5-mini-intformat & 0.80 & 1.00 & 0.00 & 0.90 & 0.95 & 0.90 \\
% gpt-5-mini-with-image & 0.70 & 0.90 & - & 0.55 & 0.95 & 0.70 \\
% gpt-oss-20b & 0.20 & 0.45 & - & 0.00 & 0.00 & 0.05 \\
% gpt-oss-20b-intformat & 0.40 & 0.85 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.10 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.15 & 0.15 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.25 & 0.65 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.30 & 0.05 & - & 0.00 & 0.00 & 0.05 \\
% olmo-3.1-32b-think-intformat & 0.50 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.25 & 0.05 & - & 0.00 & 0.05 & 0.20 \\
% qwen3-32b-intformat & 0.20 & 0.35 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-vl-235b-a22b-thinking & 0.45 & 0.60 & - & 0.00 & 0.35 & 0.25 \\
% \bottomrule
% \end{tabular}
% \end{table}
%
%
% % === MEDIUM DIFFICULTY: ACCURACY ===
%
% \begin{table}[htbp]
% \caption{Accuracy on Medium Difficulty (Verifier)}
% \label{tab:accuracy_medium_old}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.20 & 0.75 & - & 0.00 & 0.50 & 0.55 \\
% gemini-3-flash-preview & 0.60 & 0.65 & - & 0.00 & 0.05 & 0.90 \\
% gemini-3-flash-preview-intformat & 0.65 & 1.00 & - & 0.20 & 0.10 & 0.80 \\
% gemini-3-flash-preview-with-image & 0.70 & 0.50 & - & 0.00 & 0.10 & 0.95 \\
% glm-4.7-flash & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.20 & 0.75 & 0.00 & 0.00 & 0.65 & 0.85 \\
% gpt-5-mini-intformat & 0.35 & 0.80 & 0.00 & 0.10 & 0.75 & 0.60 \\
% gpt-5-mini-with-image & 0.25 & 0.70 & - & 0.00 & 0.75 & 0.80 \\
% gpt-oss-20b & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.40 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.05 & 0.20 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.05 \\
% olmo-3.1-32b-think-intformat & 0.05 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 0.05 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-vl-235b-a22b-thinking & - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \end{table}
%
%
% % === HARD DIFFICULTY: ACCURACY ===
%
% \begin{table}[htbp]
% \caption{Accuracy on Hard Difficulty (Verifier)}
% \label{tab:accuracy_hard_old}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.00 & 0.40 & - & 0.00 & 0.10 & 0.00 \\
% gemini-3-flash-preview & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.25 \\
% gemini-3-flash-preview-intformat & 0.15 & 0.75 & - & 0.00 & 0.00 & 0.40 \\
% gemini-3-flash-preview-with-image & 0.00 & 0.25 & - & 0.00 & 0.00 & 0.25 \\
% glm-4.7-flash & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.00 & 0.40 & 0.00 & 0.00 & 0.45 & 0.40 \\
% gpt-5-mini-intformat & 0.05 & 0.55 & 0.00 & 0.00 & 0.15 & 0.00 \\
% gpt-5-mini-with-image & 0.00 & 0.40 & - & 0.00 & 0.40 & 0.30 \\
% gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.10 \\
% olmo-3.1-32b-think-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-vl-235b-a22b-thinking & - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \end{table}






% ================================================================================
% OLD OLD OLD OLD OLD TABLES (One per difficulty)
% ================================================================================

% % === EASY DIFFICULTY: ACCURACY ===

% \begin{table}[htbp]
% \caption{Accuracy on Easy Difficulty (Verifier)}
% \label{tab:accuracy_easy}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.25 & 0.40 & - & 0.00 & 0.15 & 0.10 \\
% deepseek-v3.2-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview & 0.80 & 0.85 & - & 0.20 & 0.75 & 0.95 \\
% gemini-3-flash-preview-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.85 & 0.90 & - & 0.00 & 0.65 & 0.90 \\
% glm-4.7-flash & 0.05 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.80 & 0.95 & 0.00 & 0.50 & 0.95 & 0.90 \\
% gpt-5-mini-intformat & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini-with-image & 0.70 & 0.90 & - & 0.55 & 0.95 & 0.70 \\
% gpt-oss-20b & 0.20 & 0.45 & - & 0.00 & 0.00 & 0.05 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.15 & 0.15 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.30 & 0.05 & - & 0.00 & 0.00 & 0.05 \\
% olmo-3.1-32b-think-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.25 & 0.05 & - & 0.00 & 0.05 & 0.20 \\
% qwen3-32b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === MEDIUM DIFFICULTY: ACCURACY ===

% \begin{table}[htbp]
% \caption{Accuracy on Medium Difficulty (Verifier)}
% \label{tab:accuracy_medium}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.10 & 0.25 & - & 0.00 & 0.15 & 0.05 \\
% deepseek-v3.2-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview & 0.60 & 0.65 & - & 0.00 & 0.05 & 0.90 \\
% gemini-3-flash-preview-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.70 & 0.50 & - & 0.00 & 0.10 & 0.95 \\
% glm-4.7-flash & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.20 & 0.75 & 0.00 & 0.00 & 0.65 & 0.85 \\
% gpt-5-mini-intformat & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini-with-image & 0.25 & 0.70 & - & 0.00 & 0.75 & 0.80 \\
% gpt-oss-20b & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.05 \\
% olmo-3.1-32b-think-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === HARD DIFFICULTY: ACCURACY ===

% \begin{table}[htbp]
% \caption{Accuracy on Hard Difficulty (Verifier)}
% \label{tab:accuracy_hard}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% deepseek-v3.2-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.25 \\
% gemini-3-flash-preview-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.00 & 0.25 & - & 0.00 & 0.00 & 0.25 \\
% glm-4.7-flash & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini & 0.00 & 0.40 & 0.00 & 0.00 & 0.45 & 0.40 \\
% gpt-5-mini-intformat & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% gpt-5-mini-with-image & 0.00 & 0.40 & - & 0.00 & 0.40 & 0.30 \\
% gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% mercury-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% olmo-3.1-32b-think & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.10 \\
% olmo-3.1-32b-think-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}



% ================================================================================
% ADDITIONAL METRIC TABLES
% ================================================================================

% % === EASY: BOARD EXTRACTED ===

% \begin{table}[htbp]
% \caption{Board Extracted Rate - Easy Difficulty}
% \label{tab:board_exists_easy}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 1.00 & - & 1.00 & 0.95 & 0.95 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.45 & 0.35 & - & 0.30 & 0.10 & 0.20 \\
% glm-4.7-flash-intformat & 0.55 & 0.60 & - & 0.45 & 0.10 & 0.35 \\
% gpt-5-mini & 1.00 & 1.00 & 0.65 & 0.95 & 1.00 & 1.00 \\
% gpt-5-mini-intformat & 1.00 & 1.00 & 0.95 & 1.00 & 1.00 & 1.00 \\
% gpt-5-mini-with-image & 1.00 & 1.00 & - & 0.95 & 1.00 & 1.00 \\
% gpt-oss-20b & 0.20 & 0.85 & - & 0.00 & 0.00 & 0.05 \\
% gpt-oss-20b-intformat & 0.40 & 0.95 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% mercury & 0.50 & 0.50 & - & 0.15 & 0.50 & 0.45 \\
% mercury-intformat & 0.45 & 0.80 & - & 0.45 & 0.70 & 0.55 \\
% olmo-3.1-32b-think & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% olmo-3.1-32b-think-intformat & 1.00 & 1.00 & - & 1.00 & 0.95 & 1.00 \\
% qwen3-32b & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === MEDIUM: BOARD EXTRACTED ===

% \begin{table}[htbp]
% \caption{Board Extracted Rate - Medium Difficulty}
% \label{tab:board_exists_medium}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 0.95 \\
% gemini-3-flash-preview & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.15 & 0.35 & - & 0.10 & 0.00 & 0.50 \\
% glm-4.7-flash-intformat & 0.35 & 0.45 & - & 0.40 & 0.25 & 0.35 \\
% gpt-5-mini & 1.00 & 1.00 & 0.80 & 0.85 & 0.90 & 1.00 \\
% gpt-5-mini-intformat & 0.75 & 1.00 & 0.70 & 0.90 & 1.00 & 0.95 \\
% gpt-5-mini-with-image & 0.85 & 1.00 & - & 0.95 & 1.00 & 1.00 \\
% gpt-oss-20b & 0.00 & 0.30 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.60 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% mercury & 0.10 & 0.20 & - & 0.25 & 0.30 & 0.45 \\
% mercury-intformat & 0.25 & 0.55 & - & 0.45 & 0.60 & 0.55 \\
% olmo-3.1-32b-think & 1.00 & 1.00 & - & 0.75 & 1.00 & 1.00 \\
% olmo-3.1-32b-think-intformat & 0.95 & 1.00 & - & 1.00 & 1.00 & 0.75 \\
% qwen3-32b & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 1.00 & - & 1.00 & 0.95 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === HARD: BOARD EXTRACTED ===

% \begin{table}[htbp]
% \caption{Board Extracted Rate - Hard Difficulty}
% \label{tab:board_exists_hard}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 1.00 & - & 0.95 & 1.00 & 1.00 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 0.95 \\
% gemini-3-flash-preview & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.30 & 0.40 & - & 0.35 & 0.00 & 0.40 \\
% glm-4.7-flash-intformat & 0.30 & 0.30 & - & 0.30 & 0.30 & 0.65 \\
% gpt-5-mini & 0.90 & 1.00 & 0.75 & 0.90 & 0.80 & 1.00 \\
% gpt-5-mini-intformat & 0.85 & 1.00 & 0.75 & 0.90 & 0.65 & 0.95 \\
% gpt-5-mini-with-image & 0.84 & 1.00 & - & 0.95 & 0.90 & 1.00 \\
% gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% mercury & 0.10 & 0.20 & - & 0.45 & 0.15 & 0.30 \\
% mercury-intformat & 0.10 & 0.35 & - & 0.55 & 0.40 & 0.55 \\
% olmo-3.1-32b-think & 1.00 & 1.00 & - & 0.60 & 1.00 & 1.00 \\
% olmo-3.1-32b-think-intformat & 0.80 & 1.00 & - & 0.95 & 1.00 & 0.55 \\
% qwen3-32b & 1.00 & 1.00 & - & 1.00 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 1.00 & - & 1.00 & 0.95 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === EASY: BOARD STRUCTURALLY VALID ===

% \begin{table}[htbp]
% \caption{Board Structurally Valid Rate - Easy Difficulty}
% \label{tab:board_valid_easy}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 0.45 & - & 0.85 & 0.95 & 0.95 \\
% deepseek-v3.2-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% gemini-3-flash-preview & 1.00 & 0.85 & - & 0.85 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 0.90 & - & 0.90 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.30 & 0.05 & - & 0.25 & 0.05 & 0.20 \\
% glm-4.7-flash-intformat & 0.55 & 0.00 & - & 0.40 & 0.00 & 0.35 \\
% gpt-5-mini & 0.85 & 0.95 & 0.65 & 0.80 & 1.00 & 1.00 \\
% gpt-5-mini-intformat & 1.00 & 0.00 & 0.95 & 1.00 & 0.00 & 1.00 \\
% gpt-5-mini-with-image & 0.95 & 0.90 & - & 0.85 & 1.00 & 1.00 \\
% gpt-oss-20b & 0.20 & 0.75 & - & 0.00 & 0.00 & 0.05 \\
% gpt-oss-20b-intformat & 0.40 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.90 & 0.15 & - & 0.85 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% mercury & 0.45 & 0.15 & - & 0.05 & 0.30 & 0.45 \\
% mercury-intformat & 0.45 & 0.00 & - & 0.35 & 0.00 & 0.55 \\
% olmo-3.1-32b-think & 1.00 & 0.30 & - & 0.70 & 1.00 & 1.00 \\
% olmo-3.1-32b-think-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% qwen3-32b & 0.85 & 0.10 & - & 0.70 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === MEDIUM: BOARD STRUCTURALLY VALID ===

% \begin{table}[htbp]
% \caption{Board Structurally Valid Rate - Medium Difficulty}
% \label{tab:board_valid_medium}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 0.30 & - & 0.85 & 0.95 & 1.00 \\
% deepseek-v3.2-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 0.95 \\
% gemini-3-flash-preview & 1.00 & 0.75 & - & 0.95 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 0.65 & - & 0.95 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.00 & 0.05 & - & 0.05 & 0.00 & 0.50 \\
% glm-4.7-flash-intformat & 0.35 & 0.00 & - & 0.35 & 0.00 & 0.35 \\
% gpt-5-mini & 0.70 & 0.85 & 0.80 & 0.60 & 0.75 & 1.00 \\
% gpt-5-mini-intformat & 0.65 & 0.00 & 0.70 & 0.80 & 0.00 & 0.95 \\
% gpt-5-mini-with-image & 0.65 & 0.80 & - & 0.60 & 0.95 & 1.00 \\
% gpt-oss-20b & 0.00 & 0.10 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.85 & 0.00 & - & 0.50 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% mercury & 0.10 & 0.05 & - & 0.25 & 0.10 & 0.45 \\
% mercury-intformat & 0.25 & 0.00 & - & 0.30 & 0.00 & 0.55 \\
% olmo-3.1-32b-think & 0.70 & 0.05 & - & 0.45 & 0.95 & 1.00 \\
% olmo-3.1-32b-think-intformat & 0.95 & 0.00 & - & 1.00 & 0.00 & 0.75 \\
% qwen3-32b & 0.50 & 0.10 & - & 0.70 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === HARD: BOARD STRUCTURALLY VALID ===

% \begin{table}[htbp]
% \caption{Board Structurally Valid Rate - Hard Difficulty}
% \label{tab:board_valid_hard}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 1.00 & 0.10 & - & 0.65 & 1.00 & 1.00 \\
% deepseek-v3.2-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 0.95 \\
% gemini-3-flash-preview & 1.00 & 0.15 & - & 0.90 & 1.00 & 1.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% gemini-3-flash-preview-with-image & 1.00 & 0.30 & - & 0.75 & 1.00 & 1.00 \\
% glm-4.7-flash & 0.10 & 0.05 & - & 0.35 & 0.00 & 0.40 \\
% glm-4.7-flash-intformat & 0.30 & 0.00 & - & 0.20 & 0.00 & 0.65 \\
% gpt-5-mini & 0.20 & 0.55 & 0.75 & 0.70 & 0.65 & 1.00 \\
% gpt-5-mini-intformat & 0.45 & 0.00 & 0.75 & 0.65 & 0.00 & 0.95 \\
% gpt-5-mini-with-image & 0.37 & 0.55 & - & 0.95 & 0.80 & 1.00 \\
% gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.65 & 0.00 & - & 0.45 & 1.00 & 1.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 0.00 & - & 1.00 & 0.00 & 1.00 \\
% mercury & 0.05 & 0.00 & - & 0.40 & 0.00 & 0.30 \\
% mercury-intformat & 0.00 & 0.00 & - & 0.45 & 0.00 & 0.55 \\
% olmo-3.1-32b-think & 0.45 & 0.05 & - & 0.40 & 1.00 & 1.00 \\
% olmo-3.1-32b-think-intformat & 0.80 & 0.00 & - & 0.95 & 0.00 & 0.55 \\
% qwen3-32b & 0.45 & 0.00 & - & 0.50 & 1.00 & 1.00 \\
% qwen3-32b-intformat & 1.00 & 0.00 & - & 0.95 & 0.00 & 1.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === EASY: STARTING BOARD MODIFIED (ERROR) ===

% \begin{table}[htbp]
% \caption{Starting Board Modified (Error) Rate - Easy Difficulty}
% \label{tab:board_modified_easy}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.35 & 0.55 & - & 0.15 & 0.00 & 0.00 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview & 0.10 & 0.15 & - & 0.15 & 0.00 & 0.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.10 & 0.10 & - & 0.10 & 0.00 & 0.00 \\
% glm-4.7-flash & 0.25 & 0.30 & - & 0.05 & 0.05 & 0.00 \\
% glm-4.7-flash-intformat & 0.55 & 0.60 & - & 0.05 & 0.10 & 0.00 \\
% gpt-5-mini & 0.00 & 0.05 & 0.00 & 0.15 & 0.00 & 0.00 \\
% gpt-5-mini-intformat & 0.95 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% gpt-5-mini-with-image & 0.05 & 0.10 & - & 0.10 & 0.00 & 0.00 \\
% gpt-oss-20b & 0.00 & 0.10 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.40 & 0.95 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 1.00 & 0.85 & - & 0.15 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% mercury & 0.05 & 0.35 & - & 0.10 & 0.20 & 0.00 \\
% mercury-intformat & 0.35 & 0.80 & - & 0.10 & 0.70 & 0.00 \\
% olmo-3.1-32b-think & 0.40 & 0.70 & - & 0.30 & 0.00 & 0.00 \\
% olmo-3.1-32b-think-intformat & 0.95 & 1.00 & - & 0.00 & 0.95 & 0.00 \\
% qwen3-32b & 0.40 & 0.90 & - & 0.30 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === MEDIUM: STARTING BOARD MODIFIED (ERROR) ===

% \begin{table}[htbp]
% \caption{Starting Board Modified (Error) Rate - Medium Difficulty}
% \label{tab:board_modified_medium}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.65 & 0.70 & - & 0.15 & 0.05 & 0.00 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview & 0.15 & 0.25 & - & 0.05 & 0.00 & 0.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.20 & 0.35 & - & 0.05 & 0.00 & 0.00 \\
% glm-4.7-flash & 0.10 & 0.30 & - & 0.05 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.35 & 0.45 & - & 0.05 & 0.25 & 0.00 \\
% gpt-5-mini & 0.15 & 0.15 & 0.00 & 0.25 & 0.15 & 0.00 \\
% gpt-5-mini-intformat & 0.65 & 1.00 & 0.00 & 0.10 & 1.00 & 0.00 \\
% gpt-5-mini-with-image & 0.10 & 0.20 & - & 0.35 & 0.05 & 0.00 \\
% gpt-oss-20b & 0.00 & 0.20 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.60 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 1.00 & 1.00 & - & 0.50 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% mercury & 0.10 & 0.15 & - & 0.00 & 0.20 & 0.00 \\
% mercury-intformat & 0.20 & 0.55 & - & 0.15 & 0.60 & 0.00 \\
% olmo-3.1-32b-think & 0.65 & 0.95 & - & 0.30 & 0.05 & 0.00 \\
% olmo-3.1-32b-think-intformat & 0.90 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% qwen3-32b & 0.75 & 0.90 & - & 0.30 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 1.00 & 1.00 & - & 0.00 & 0.95 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}


% % === HARD: STARTING BOARD MODIFIED (ERROR) ===

% \begin{table}[htbp]
% \caption{Starting Board Modified (Error) Rate - Hard Difficulty}
% \label{tab:board_modified_hard}
% \begin{tabular}{lrrrrrr}
% \toprule
% model & FlowFree & Bridges & Loopy & Galaxies & Undead & Pattern \\
% \midrule
% deepseek-v3.2 & 0.90 & 0.90 & - & 0.30 & 0.00 & 0.00 \\
% deepseek-v3.2-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview & 0.60 & 0.85 & - & 0.10 & 0.00 & 0.00 \\
% gemini-3-flash-preview-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% gemini-3-flash-preview-with-image & 0.70 & 0.70 & - & 0.25 & 0.00 & 0.00 \\
% glm-4.7-flash & 0.20 & 0.35 & - & 0.00 & 0.00 & 0.00 \\
% glm-4.7-flash-intformat & 0.25 & 0.30 & - & 0.10 & 0.30 & 0.00 \\
% gpt-5-mini & 0.00 & 0.45 & 0.00 & 0.20 & 0.15 & 0.00 \\
% gpt-5-mini-intformat & 0.30 & 1.00 & 0.00 & 0.25 & 0.65 & 0.00 \\
% gpt-5-mini-with-image & 0.05 & 0.45 & - & 0.00 & 0.10 & 0.00 \\
% gpt-oss-20b & 0.00 & 0.00 & - & 0.00 & 0.00 & 0.00 \\
% gpt-oss-20b-intformat & 0.00 & 0.05 & - & 0.00 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct & 0.95 & 1.00 & - & 0.55 & 0.00 & 0.00 \\
% llama-4-maverick-17b-128e-instruct-intformat & 1.00 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% mercury & 0.05 & 0.20 & - & 0.05 & 0.15 & 0.00 \\
% mercury-intformat & 0.00 & 0.35 & - & 0.10 & 0.40 & 0.00 \\
% olmo-3.1-32b-think & 0.70 & 0.95 & - & 0.20 & 0.00 & 0.00 \\
% olmo-3.1-32b-think-intformat & 0.70 & 1.00 & - & 0.00 & 1.00 & 0.00 \\
% qwen3-32b & 0.75 & 1.00 & - & 0.50 & 0.00 & 0.00 \\
% qwen3-32b-intformat & 0.85 & 1.00 & - & 0.05 & 0.95 & 0.00 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> todo.tex <==





\section{TODO}

TopoBench
LLMs find it hard to solve 2d grid puzzles because of representation and state explosion/tracking !

1. Literature review of existing puzzles-- how they differ from ours 
2. Big table for main results. -- finish this by end of this week 
    a. loopy put a border around loopy! (remember empty line at start and end) and also check prompt again. („Do not ask questions, solve the puzzle with the information you have“) It's ok if loopy stays very hard, but it can't be zero for every model. (Nils)
    b. IS it possible to do the cot intervention with lm or just with the verifier game trees?
    c. New type of analysis: can we convert cot into game tree for easier analysis?
    
3. Analysis of why models find it hard. -- 
    0. search for ways to do the analysis in other papers (Nils) (why are models failing?)
    a. representation
        i. tokenization analysis (tiktokenizer for gpt models)
    b. state -- 
        i. context rot -- blocker - we need good open source cot--
        ii. another approach -- solver state till a point and ask model to solve, vs solver state + k junk states till a point and ask model to solve (Janak)
        iii. Does having a gt representation of a state outside of the model help? -- tool- call thing with bridges in ascii -- not images--(Janak)
    c. search -- 
        i. Do models explore new branches or do they get stuck?
        ii. Run model multiple times and see if it explores different areas
        iii. Can we compare a reasoning model with a reasoning model? (maybe do a pass@highnumber)
        iiii. Comparison to gpt5-mini-low? (Do models reason differently when adjusting reasoning effort?)
    d. cursor based analysis of cot logs, create reports, verify and post on channel (Janak, Nils) -- find more analysis axes from this ! 
4. Barebones version of the paper! -
5. Finetuning Results 
    a. rsft and grpo
    b. tokenization, architecture changes! 



state: guide experiments by error analysis (prompt with possible errors)
1) make mistake, then solve from there


Questions:
Can weak models solve puzzles when given the (summarised) cots of a strong one?
Can we change the adjacency matrix (ProsQA) experiment to make sense? (maybe with bridges solution tree? - we would need a full solver first)
Do newline characters give models a sense of spatial relations?: Can models understand spatial relations in ascii (“which character is under the U”)?
Can models convert to different formats?
Con models reconstruct the startboard from the cot if we remove it?
Can we separate length of cot from difficulty?


30th January 

Todo for iclr workshop experiments

Experiments
0. Figure out partial game trees from bridges c code -- Mayug 
1. Error Analysis  -- histogram plot; 
    a. Look at other papers for error analysis -- kore gym, illusion of thinking, a ffew of the benchmarking ones
2. Intformat-json full experiments -- Nils -- prompts and rerun
2. State -- Interventions
3. Externalizing State -- tool call -- Janak
4. Loopy -- Nils with border  
5. Representation - Tokenizer Analysis
6. Qwen3-70B pass@8 b/w instruction tuned and rl tuned (last)
7. Deepseek v3.2 Reasoner -- for RFT , also give soln path and ask it to solve in an alternate way 
8. Toy experiment -- Mayug, today or tomorrow !! 
9. Introduction -- Put it in the intro for now ! -for puzzle selection !! -- Puzzle selection setup, 


Writing



Outline brainstorming 

Large language models frequently fail on grid and topology puzzles that demand iterative state updates over a structured representation. We present Topo-Bench, a suite of verifiable grid/topological puzzles across six families, three difficulty tiers, and diverse encodings (ASCII, integer grids, JSON, and image+text). On the hardest tier, leading closed-source models attain low pass rates (0.25 for GPT-5-mini-high; 0.10 for Gemini-3-Flash), while open-source models are near zero. We show that these failures are driven less by “reasoning depth” than by the representation interface: minor encoding changes cause large, non-monotonic accuracy swings, and convert-then-solve approaches often degrade performance relative to solving in a stable encoding. To explain why, we analyze tokenizer behavior and find that common ASCII grid formats tokenize into uneven, staggered cell boundaries, whereas integer-JSON encodings yield more uniform, cell-aligned tokenization, correlating with higher accuracy across both closed- and open-source models. Finally, controlled state corruption tests (inconsistent intermediate states; frozen grid updates) induce sharp accuracy drops, revealing compounding errors from brittle state maintenance. Our findings argue that progress on visual-thinking requires optimizing not only models and training, but also the representation and state-update channels they must operate over.


How is it different from other similar benchmarks?
-very long cot reasoning
-harder
-in context reasoning, not verifiers

How is topological reasoning different from spatial reasoning?


V1 
Introduce topo and spatial reasoning, benchmarks related to spatial reasoning
topo not properly evaluated ...


Topological Reasoning 
-we define it as being about connections?


Illustrative figure showing what capabilities we are testing compared to the capabilities other benchmarks are testing 

we refer to this and talk about connectivity, symmetry, other topological stuff, holes, 

we need a benchmark for this 

why would llms getting better on topological reasoning matter? -- humans can do 9x9 puzzle in 5 mins but llms cant, 
because geometrical reasoning, requires state maintenance, requires reasoning long cot 



outline 2



show visual 

toy experiments (isomorphism / complexity like) -- control for complexity and do the graye aph for an llm 
-> visual puzzle should be hard and text equivalent easy for llm (maybe from "illusion of thinking"

6 puzzles -- non visual -- algebraic one, word puzzles,  -- no need if toy experiment !! 


correlation between puzzle performance and geometry math, algebra math

Spatial Reasoning 


Main question still: how did we choose the puzzles? 
-find list of visual criteria for visual load, then use llm to classify puzzles (manually verify them)

-SGR category is lowest in https://arxiv.org/html/2505.14552v2 korgym
so we want to focus on higher visual load puzzles.

Workshop outline (6–8 pages)
Intro + claim (representation bottleneck)
Benchmark (puzzle families, difficulty tiers, verifiers, representations)
Main results: representation sweep + convert-then-solve vs solve-directly
Mini causal analysis: context pollution experiments (2–3 interventions)
Discussion + limitations + future work (sets up training story)



Interventions: -- 
